Generating 3D Binding Molecules Using Shape-Conditioned Diffusion Models with Guidance

Drug development is a critical but notoriously resource- and time-consuming process. In this manuscript, we develop a novel generative artificial intelligence (genAI) method DiffSMol to facilitate drug development. DiffSmol generates 3D binding molecules based on the shapes of known ligands. DiffSMol encapsulates geometric details of ligand shapes within pre-trained, expressive shape embeddings and then generates new binding molecules through a diffusion model. DiffSMol further modifies the generated 3D structures iteratively via shape guidance to better resemble the ligand shapes. It also tailors the generated molecules toward optimal binding affinities under the guidance of protein pockets. Here, we show that DiffSMol outperforms the state-of-the-art methods on benchmark datasets. When generating binding molecules resembling ligand shapes, DiffSMol with shape guidance achieves a success rate 61.4%, substantially outperforming the best baseline (11.2%), meanwhile producing molecules with novel molecular graph structures. DiffSMol with pocket guidance also outperforms the best baseline in binding affinities by 13.2%, and even by 17.7% when combined with shape guidance. Case studies for two critical drug targets demonstrate very favorable physicochemical and pharmacokinetic properties of the generated molecules, thus, the potential of DiffSMol in developing promising drug candidates.

==> algorithms/train_diff.tex <==
\begin{algorithm}[!h]
    \caption{Training Procedure of \methoddiff}
    \label{alg:diffgen}
    \begin{algorithmic}[1]
        \Require $\shapehiddenmat, \molx, \pocket$
        \FullLineComment{sample the number of atoms in the generated molecule}
    \end{algorithmic}
\end{algorithm}

==> algorithms/train_se.tex <==
\begin{algorithm}[!h]
    \caption{Training Procedure of \SE}
    \label{alg:diffgen}
    \begin{algorithmic}[1]
        \Require $\shapehiddenmat, \molx, \pocket$
        \FullLineComment{sample the number of atoms in the generated molecule}
    \end{algorithmic}
\end{algorithm}

==> tables/ablation_study_desirable.tex <==
\begin{table*}[h]
	\centering
		\caption{Comparison on Desirable Molecules for SMG}
	\label{tbl:ablation_study_desirable}
\begin{threeparttable}
	\begin{scriptsize}
	\begin{tabular}{
		%
		@{\hspace{3pt}}l@{\hspace{3pt}}
		%
		@{\hspace{3pt}}r@{\hspace{8pt}}
		@{\hspace{3pt}}c@{\hspace{3pt}}
		@{\hspace{3pt}}r@{\hspace{3pt}}
		%
		@{\hspace{4pt}}c@{\hspace{4pt}}
		%
		@{\hspace{3pt}}r@{\hspace{3pt}}
		@{\hspace{3pt}}c@{\hspace{3pt}}
		@{\hspace{3pt}}r@{\hspace{3pt}}
		%
		@{\hspace{4pt}}c@{\hspace{4pt}}
		%
		@{\hspace{3pt}}r@{\hspace{3pt}}
		@{\hspace{3pt}}c@{\hspace{3pt}}
		@{\hspace{3pt}}r@{\hspace{3pt}}
		%
		@{\hspace{4pt}}c@{\hspace{4pt}}
		%
		@{\hspace{3pt}}r@{\hspace{3pt}}
		@{\hspace{3pt}}c@{\hspace{3pt}}
		@{\hspace{3pt}}r@{\hspace{3pt}}
		%
		%@{\hspace{3pt}}r@{\hspace{3pt}}
		}
		\toprule
		\multirow{2}{*}{method}  & \multicolumn{3}{c}{$\delta_g$=0.3} & & \multicolumn{3}{c}{$\delta_g$=0.5} & & \multicolumn{3}{c}{$\delta_g$=0.7} & & \multicolumn{3}{c}{$\delta_g$=1.0}  \\
		\cmidrule{2-4} \cmidrule{6-8} \cmidrule{10-12} \cmidrule{14-16}
		%
		& \desire & \diversity & \novel & & \desire & \diversity & \novel & &  \desire & \diversity & \novel & & \desire & \diversity & \novel \\ 
		\midrule
		%\dataset &  10.6     & 0.736         &  0.0 & & 12.2            & 0.734 & 0.0 &  &  12.3 & 0.734 &  0.0 & &  12.3 & 0.734 & 0.0 \\
		\method               &  \underline{28.4}    & \textbf{0.762} & \underline{99.8} & &  \underline{32.3}    & \textbf{0.751} & \underline{99.8} & &  \underline{32.4}    & \textbf{0.751} & \underline{99.8}  &  &  \underline{32.4}    & \textbf{0.751}   & \underline{99.8}  \\
		\methodwithsguide     & \textbf{61.4}   & \underline{0.760}   & \textbf{99.9} & & \textbf{70.9}   & \underline{0.748}   & \textbf{99.9} & &  \textbf{71.0}   & \underline{0.748}  & \textbf{99.9}  &  &  \textbf{71.0}   & \underline{0.748}   & \textbf{99.9}  \\
		\midrule
		\method (EGNN) & 11.0   & 0.743 & 99.8 & & 12.4 & 0.734 & 99.8 & & 12.4 & xxx & 99.8 & & 12.4 & xxx & 99.8 \\
		\method (no bond) & 28.6   & 0.765 & 99.8 & & 32.4 & 0.756 & 99.8 & & 32.5 & xxx & 99.8 & & 32.5 & xxx & 99.8 \\
		\method (no shape) & 0.9   & 0.793 & 100.0 & & 1.0 & 0.793 & 100.0 & & 1.0 & xxx & 100.0 & & 1.0 & xxx & 100.0 \\
	\bottomrule
	\end{tabular}%
	\begin{tablenotes}[normal,flushleft]
		\begin{footnotesize}
	\item 
\!\!Columns represent: {``$\delta_g$'': the graph similarity constraint; 
``\desire'': the percentage of generated molecules that are desirable, satisfying $\delta_g$ and exhibiting high \shapesim ($\shapesim>=0.8$);
``\diversity'': the diversity among the desirable molecules;
``\novel'': the percentage of desirable molecules that cannot be found in the MOSES dataset.
%
%``$\uparrow$'' represents higher values are better, and ``$\downarrow$'' represents lower values are better.
%
 Best values are in \textbf{bold}, and second-best values are \underline{underlined}. 
} 
\par
		\par
		\end{footnotesize}
	\end{tablenotes}
	\end{scriptsize}
\end{threeparttable}
\end{table*}


==> tables/ablation_study_quality.tex <==
\begin{table*}[!h]
	\centering
		\caption{Ablation Study Comparison on Quality of Generated Desirable Molecules ($\delta$=0.3)}
	\label{tbl:ablation_study_quality}
	\begin{scriptsize}
\begin{threeparttable}
	\begin{tabular}{
		@{\hspace{0pt}}l@{\hspace{14pt}}
		@{\hspace{0pt}}l@{\hspace{2pt}}
		%
		@{\hspace{4pt}}c@{\hspace{4pt}}
		%
		%@{\hspace{3pt}}c@{\hspace{3pt}}
		@{\hspace{3pt}}c@{\hspace{3pt}}
		@{\hspace{3pt}}c@{\hspace{3pt}}
		@{\hspace{3pt}}c@{\hspace{3pt}}
		@{\hspace{3pt}}c@{\hspace{3pt}}
		@{\hspace{3pt}}c@{\hspace{3pt}}
		%
		%
		}
		\toprule
		group & metric & 
        %& \dataset 
        &  \method & \methodwithsguide & \method egnn & \method no bond & \method no shape \\
		%\multirow{2}{*}{method} & \multirow{2}{*}{\#c\%} &  \multirow{2}{*}{\#u\%} &  \multirow{2}{*}{QED} & \multicolumn{3}{c}{$\nmax=50$} & & \multicolumn{2}{c}{$\nmax=1$}\\
		%\cmidrule(r){5-7} \cmidrule(r){8-10} 
		%& & & & \avgshapesim(std) & \avggraphsim(std  &  \diversity(std  & & \avgshapesim(std) & \avggraphsim(std \\
		\midrule
		\multirow{2}{*}{stability}
		& atom stability ($\uparrow$) & 
        %& 0.990 
        & \textbf{0.993} & \textbf{0.989} & 0.939 & 0.979 & 0.933     \\
		& mol stability ($\uparrow$) & 
        %& 0.876 
        & 0.891 & 0.850 & 0.314 & 0.714 & 0.310    \\
		\midrule
	%	\multirow{3}{*}{Drug-likeness} 
	%	& QED ($\uparrow$) & 
        %& \textbf{0.805} 
        %& \textbf{0.766} & 0.760 & 0.755 & 0.751    \\
	%	& SA ($\uparrow$) & 
        %& \textbf{0.874} 
        %& \textbf{0.813} & \textbf{0.813} & 0.699 & 0.692    \\
	%	& Lipinski ($\uparrow$) & 
        %& \textbf{4.999} 
        %& 4.979 & \textbf{4.980} & 4.967 & 4.975    \\
	%	\midrule
		\multirow{4}{*}{3D structures} 
		& RMSD ($\downarrow$) & 
        %& \textbf{0.420} 
        & 0.895 & 0.882 & - & - & -    \\
		& JS. bond lengths ($\downarrow$) & 
        %& \textbf{0.286} 
        & 0.438 & 0.431 & 0.529 & \textbf{0.388} & 0.407   \\
		& JS. bond angles ($\downarrow$) & 
        %& \textbf{0.078} 
        & \textbf{0.185} & 0.199 & 0.293 & 0.193 & 0.250   \\
		& JS. dihedral angles ($\downarrow$) & 
        %& \textbf{0.151} 
        & \textbf{0.168} & 0.170 & 0.244 & 0.197 & 0.226    \\
		\midrule
		\multirow{5}{*}{2D structures} 
		& JS. \#bonds per atoms ($\downarrow$) & 
        %& 0.325 
        & 0.176 & \textbf{0.172} & 0.186 & 0.230 & 0.178    \\
		& JS. basic bond types ($\downarrow$) & 
        %& \textbf{0.055} 
        & \textbf{0.180} & 0.190 & 0.273 & 0.189 & 0.207   \\
	%	& JS. freq. bond types ($\downarrow$) & 
        %& \textbf{0.089} 
        %& \textbf{0.123} & 0.130 & 0.245 & 0.254    \\
	%	& JS. freq. bond pairs ($\downarrow$) & 
        %& \textbf{0.078} 
        %& \textbf{0.085} & 0.089 & 0.209 & 0.221    \\
	%	& JS. freq. bond triplets ($\downarrow$) & 
        %& \textbf{0.089} 
        %& \textbf{0.097} & 0.114 & 0.211 & 0.223    \\
		%\midrule
		%\multirow{3}{*}{Rings} 
		& JS. \#rings ($\downarrow$) & 
        %& 0.143 
        & \textbf{0.042} & 0.048 & 0.058 & 0.158 & 0.098    \\
		& JS. \#n-sized rings ($\downarrow$) & 
        %& \textbf{0.055} 
        & \textbf{0.098} & 0.111 & 0.106 & 0.101 & 0.114    \\
		& \#Intersecting rings ($\uparrow$) & 
        %& \textbf{6} 
        & 4 & \textbf{5} & 4 & \textbf{5} & 4   \\
		%\method (+bt)            & 100.0 & 98.0 & 100.0 & 0.742 & 0.772 (0.040) & 0.211 (0.033) & & 0.862 (0.036) & 0.211 (0.033) & 0.743 (0.043) \\
		%\methodwithguide (+bt)    & 99.8 & 98.0 & 100.0 & 0.736 & 0.814 (0.031) & 0.193 (0.042) & & 0.895 (0.029) & 0.193 (0.042) & 0.745 (0.045) \\
		%
		\bottomrule
	\end{tabular}%
	\begin{tablenotes}[normal,flushleft]
		\begin{footnotesize}
	\item 
\!\!Rows represent:  {``atom stability'': the proportion of stable atoms that have the correct valency; 
		``molecule stability'': the proportion of generated molecules with all atoms stable;
		%``QED'': the drug-likeness score;
		%``SA'': the synthesizability score;
		%``Lipinski'': the Lipinski 
		``RMSD'': the root mean square deviation (RMSD) between the generated 3D structures of molecules and their optimal conformations; % identified via energy minimization;
		``JS. bond lengths/bond angles/dihedral angles'': the Jensen-Shannon (JS) divergences of bond lengths, bond angles and dihedral angles;
		``JS. \#bonds per atom/basic bond types/\#rings/\#n-sized rings'': the JS divergences of bond counts per atom, basic bond types, counts of all rings, and counts of n-sized rings;
		%``JS. \#rings/\#n-sized rings'': the JS divergences of the total counts of rings and the counts of n-sized rings;
		``\#Intersecting rings'': the number of rings observed in the top-10 frequent rings of both generated and real molecules. } \par
		\par
		\end{footnotesize}
	\end{tablenotes}
\end{threeparttable}
\end{scriptsize}
\end{table*}


==> tables/ablation_study_results.tex <==
\begin{table*}
	\centering
		\caption{Ablation Study}
	\label{tbl:ablation_study}
	\begin{small}
\begin{threeparttable}
	\begin{tabular}{
		@{\hspace{0pt}}l@{\hspace{2pt}}
		%
		@{\hspace{5pt}}r@{\hspace{5pt}}
		@{\hspace{5pt}}r@{\hspace{5pt}}
		@{\hspace{5pt}}r@{\hspace{5pt}}
		@{\hspace{5pt}}r@{\space{5pt}}
		%
		%
		@{\hspace{5pt}}r@{\hspace{5pt}}
		%
		@{\hspace{5pt}}r@{\hspace{5pt}}
		%
		@{\hspace{0pt}}c@{\hspace{0pt}}
		%
	    	@{\hspace{5pt}}c@{\hspace{5pt}}
		%
		@{\hspace{5pt}}c@{\hspace{5pt}}
		%
		@{\hspace{5pt}}c@{\hspace{3pt}}
		%
		}
		\toprule
		method & \#v\% & \#s\% & \#u\%  & \qed  & \avgshapesim(std) & \avggraphsim(std) & & \maxshapesim(std) & \maxgraphsim(std) &  \diversity(std) \\
		%\multirow{2}{*}{method} & \multirow{2}{*}{\#c\%} &  \multirow{2}{*}{\#u\%} &  \multirow{2}{*}{QED} & \multicolumn{3}{c}{$\nmax=50$} & & \multicolumn{2}{c}{$\nmax=1$}\\
		%\cmidrule(r){5-7} \cmidrule(r){8-10} 
		%& & & & \avgshapesim(std) & \avggraphsim(std  &  \diversity(std  & & \avgshapesim(std) & \avggraphsim(std \\
		\midrule
		\method                              & 99.6 & 98.8 & 100.0 & 0.748 & 0.689 (0.044) & 0.239 (0.049) & & 0.803 (0.042) & 0.243 (0.068) & 0.712 (0.055) \\
		\methodwithguide               & 99.6 & 98.7 & 100.0 & 0.749 & 0.746 (0.036) & 0.241 (0.050) & & 0.852 (0.034) & 0.247 (0.068) & 0.703 (0.053) \\
		\method with EGNN           & 97.3 & 97.3  & 
		%
		\bottomrule
	\end{tabular}%
	\begin{tablenotes}[normal,flushleft]
		\begin{footnotesize}
	\item 
\!\!Columns represent: \ziqi{``\#v\%'': the percentage of valid molecules; ``\#s\%'': the percentage of valid and connected molecules;}%``\#c\%": the percentage of connected molecules; 
``\#u\%'': the percentage of unique molecules;
``\qed'': the average drug-likeness of generated molecules;
``\avgshapesim/\avggraphsim'': the average of shape or graph similarities between the condition molecules and generated molecules; ``std": the standard deviation;
``\maxshapesim'': the maximum of shape similarities between the condition molecules and generated molecules;
``\maxgraphsim'': the graph similarities between the condition molecules and the molecules with the maximum shape similarities;
``\diversity'': the diversity among the generated molecules. \par
		\par
		\end{footnotesize}
	\end{tablenotes}
\end{threeparttable}
\end{small}
  \vspace{-10pt}    
\end{table*}


==> tables/ablation_study_shapeguidance.tex <==
\begin{table}[!t]
	\centering
		\caption{{Parameter Study in Shape Guidance}}
	\label{tbl:ablation_study:shape_guidance}
	\begin{small}
\begin{threeparttable}
	\begin{tabular}{
		%@{\hspace{2pt}}l@{\hspace{2pt}}
		@{\hspace{2pt}}r@{\hspace{3pt}}
		@{\hspace{3pt}}r@{\hspace{3pt}}
		%
		@{\hspace{2pt}}r@{\hspace{2pt}}
		@{\hspace{2pt}}r@{\hspace{2pt}}
		%@{\hspace{2pt}}r@{\hspace{3pt}}
		%@{\hspace{2pt}}r@{\hspace{2pt}}
		@{\hspace{2pt}}r@{\hspace{2pt}}
		%
		@{\hspace{0pt}}r@{\hspace{0pt}}
		%
		@{\hspace{2pt}}r@{\hspace{0pt}}
		@{\hspace{0pt}}r@{\hspace{2pt}}
		%
		@{\hspace{0pt}}c@{\hspace{0pt}}
		%
	    	@{\hspace{2pt}}c@{\hspace{2pt}}
		@{\hspace{2pt}}c@{\hspace{2pt}}
		%
		}
		\toprule
		% \multirow{2}{*}{$r$}  &  \multirow{2}{*}{$S$}  & \multirow{2}{*}{\#c\%} &  \multirow{2}{*}{\#u\%} &  \multirow{2}{*}{QED} &  %\multirow{2}{*}{SA} &  
		% \multirow{2}{*}{JS. bond} & & \multicolumn{2}{c}{$\nmax=1$} & & \multicolumn{2}{c}{$\nmax=50$}\\
		%\cmidrule(r){8-9} \cmidrule(r){11-12}
		%method & 
		$\gamma$ & $S$ & \qed & JS. bond & & \avgshapesim & \avggraphsim  & & \maxshapesim & \maxgraphsim  \\
		\midrule
		%\dataset                                & - & - & 100.0\% & 100.0\% & - & - & - & & 0.807 (0.042 & 0.241 (0.087 & & 0.729 (0.039 & 0.226 (0.038 \\
		%\squid ($\lambda$=1.0)        & - & - & 100.0\% &   95.0\% & 0.760 & 0.813 & - & & 0.842 (0.061 & 0.271 (0.096 & & 0.670 (0.069 & 0.235 (0.045 \\
		%\method (w/o \regularizer)    & 
		%\method & 
		- & - &  0.748 & %0.673 & 
		0.094  & & 0.689  & 0.239  & & 0.803 & 0.243 \\
		\midrule
		%\method                                & 
		%	\multirow{12}{*}{\rotatebox[origin=c]{90}{\parbox[c]{5cm}{\centering \methodwithguide}}} 
			%\multirow{9}{*}{\methodwithguide}
		0.2 & 50 &  0.630 & %0.607 & 
		0.110 & & 0.794 & 0.236 & & 0.890 & 0.244 \\
		%\method                                &  
		0.2 & 100 &  0.666 & %0.616 & 
		0.105 & & 0.786  & 0.238  & & 0.883  & 0.245  \\
		%\method                                &  
		0.2 & 300 &  0.749 & %0.656 & 
		0.093 & & 0.746  & 0.241 & & 0.852 & 0.247  \\
		%\method                                &  
%		& 0.2 & 500 & 98.9 &  0.755 & %0.676 & 
%		0.091 & & 0.694 (0.039) & 0.241 (0.048) & & 0.811 (0.039) & 0.244 (0.066) \\
		\cmidrule{1-10}
		%\method                                & 
		0.4 & 50 &  0.678 & %0.616 & 
		0.106  & & 0.779 & 0.240  & & 0.875  & 0.245  \\
		%\method                                & 
		0.4 & 100 &  0.700 & %0.625 & 
		0.103 & & 0.772  & 0.241 & & 0.870 & 0.247  \\
		%\method                                & 
		0.4 & 300 &  0.752 & %0.659 & 
		0.093 & & 0.738  & 0.242 & & 0.845 & 0.247  \\
%		& 0.4 & 500 & 98.9 &  0.756 & %0.676 & 
%		0.091 & &  0.693 (0.039) & 0.241 (0.048) & & 0.810 (0.040) & 0.245 (0.065) \\
		\cmidrule{1-10}
		%\method                               & 
		0.6 & 50 &  0.706 & %0.624 & 
		0.103  & & 0.763  & 0.242  & & 0.861  & 0.246  \\
		%\method                                & 
		0.6 & 100 &  0.720 & %0.632 & 
		0.100 & & 0.758  & 0.242  & & 0.857  & 0.247  \\
		%\method                                & 
		0.6 & 300 &  0.753 & %0.660 & 
		0.093 & & 0.731  & 0.242  & & 0.838  & 0.247  \\
%		& 0.6 & 500 & 98.9 &  0.755 & %0.676 & 
%		0.091 & & 0.691 (0.039) & 0.241 (0.048) & & 0.808 (0.040) & 0.244 (0.065) \\
	\bottomrule
	\end{tabular}%
	\begin{tablenotes}[normal,flushleft]
		\begin{footnotesize}
	\item 
\!\!Columns represent: ``$\gamma$''/``$S$'': distance threshold/step threshold in shape guidance;
%``\#c\%": the percentage of connected molecules; ``\#u\%'': the percentage of unique molecules;
%``\qed'': the average drug-likeness of generated molecules;
``JS. bond'': the JS divergence of bond length distributions of all the bond types between real molecules and generated molecules;
%``\avgshapesim/\avggraphsim'': the average of shape or graph similarities between the condition molecule and generated molecules; ``std": the standard deviation; 
%``\maxshapesim'': the maximum of shape similarities between the condition molecules and generated molecules;
%``\maxgraphsim'': the graph similarities between the condition molecules and the molecules with the maximum shape similarities. 
All the others are identical to those in Table~\ref{tbl:overall}. \par
		\par
		\end{footnotesize}
	\end{tablenotes}
\end{threeparttable}
\end{small}
  \vspace{-15pt}    
\end{table}


==> tables/ablation_study_timestepweight.tex <==
\begin{table}
	\centering
		\caption{Comparison of Diffusion Weighting Schemes}
	\label{tbl:ablation_study:timestepweight}
	\begin{small}
\begin{threeparttable}
%	\setlength\tabcolsep{0pt}
	\begin{tabular}{
		@{\hspace{3pt}}l@{\hspace{0pt}}
		%
		@{\hspace{3pt}}c@{\hspace{3pt}}
		%
		@{\hspace{3pt}}r@{\hspace{3pt}}
		@{\hspace{3pt}}r@{\hspace{3pt}}
		@{\hspace{3pt}}r@{\hspace{3pt}}
		%
		@{\hspace{3pt}}r@{\hspace{3pt}}
		%
		@{\hspace{6pt}}r@{\hspace{3pt}}
		%
%		@{\hspace{3pt}}c@{\hspace{3pt}}
		%
%		@{\hspace{3pt}}c@{\hspace{3pt}}
		%
		@{\hspace{3pt}}c@{\hspace{3pt}}
		}
		\toprule
		\multirow{2}{*}{method} & \multirow{2}{*}{weights} & \multirow{2}{*}{\#v\%}  & \multirow{2}{*}{\#s\%} & \multirow{2}{*}{\#u\%} &\multirow{2}{*}{\qed} & \multicolumn{2}{c}{JS divergence}\\
		\cmidrule(r){7-8}
		& & & &  & & bond & C-C\\
		\midrule
		\multirow{2}{*}{\method}  & \\
		& \\
		%\multirow{2}{*}{\method}   & $w^{\mathtt{x}}_t$ & 99.6 & 98.8 & 100.0 & 0.748 & %0.673 & 
%		0.106 & 0.095 &  0.321 \\
		% 0.095 &  0.321 \\
		%&   uniform   & 99.2 & 89.4 & 100.0 & 0.660 & %0.636 & 
%		0.105 & 0.115 & 0.393 \\
		%0.115 & 0.393 \\
		\midrule
		\multirow{2}{*}{\methodwithsguide} & \\
		& \\
		%\multirow{2}{*}{\methodwithguide} & $w^{\mathtt{x}}_t$  & 99.6 & 98.7 & 100.0 & 0.749 & %0.656 & 
%		0.114 & 0.093 & 0.317 \\
		%0.093 & 0.317 \\
		%&   uniform   & 99.1 & 90.1 & 100.0 & 0.671 & %0.635 & 
%		0.112 & 0.112 & 0.384 \\
		%0.112 & 0.384 \\
		\bottomrule
	\end{tabular}%
	%
	\begin{tablenotes}[normal,flushleft]
		\begin{footnotesize}
	\item 
\!\!Columns represent: 
%``\#c\%": the percentage of connected molecules; ``\#u\%'': the percentage of unique molecules;
%``\qed'': the average drug-likeness of generated molecules;
``weights": different weighting schemes;
``JS distance of bond/C-C'': the Jensen-Shannon (JS) divergence of bond length among all the bond types (``bond")/carbon-carbon single bonds (``C-C") between real molecules and generated molecules; 
All the others are identical to those in Table~\ref{tbl:overall}. 
		\par
		\end{footnotesize}
	\end{tablenotes}
\end{threeparttable}
\end{small}
\end{table}


==> tables/binding_generated_mols.tex <==
\begin{table*}
	\centering
		\caption{Drug Properties of Generated Molecules}
	\label{tbl:binding_drug_mols}
	\begin{scriptsize}
\begin{threeparttable}
	\begin{tabular}{
		@{\hspace{6pt}}r@{\hspace{6pt}}
		@{\hspace{6pt}}r@{\hspace{6pt}}
		@{\hspace{6pt}}r@{\hspace{6pt}}
		@{\hspace{6pt}}r@{\hspace{6pt}}
		@{\hspace{6pt}}r@{\hspace{6pt}}
		@{\hspace{6pt}}r@{\hspace{6pt}}
		@{\hspace{6pt}}r@{\hspace{6pt}}
		@{\hspace{6pt}}r@{\hspace{6pt}}
		@{\hspace{6pt}}r@{\hspace{6pt}}
		%
		}
		\toprule
Target & Molecule & Vina S & Vina M & Vina D & QED   & SA   & Logp  & Lipinski \\
\midrule
\multirow{3}{*}{CDK6} & NL-001 & -6.817      & -7.251    & -8.319     & 0.834 & 0.72 & 1.313 & 5        \\
& NL-002 & -6.970       & -7.605    & -8.986     & 0.851 & 0.74 & 3.196 & 5        \\
\cmidrule{2-9}
& 4AU & 0.736       & -5.939    & -7.592     & 0.773 & 0.79 & 2.104 & 5        \\
\midrule
\multirow{2}{*}{NEP} & NL-003 & -11.953     & -12.165   & -12.308    & 0.772 & 0.57 & 2.944 & 5        \\
\cmidrule{2-9}
& BIR & -9.399      & -9.505    & -9.561     & 0.463 & 0.73 & 2.677 & 5        \\
		\bottomrule
	\end{tabular}%
	\begin{tablenotes}[normal,flushleft]
		\begin{footnotesize}
	\item Columns represent: {``Target'': the names of protein targets;
		``Molecule'': the names of generated molecules and known ligands;
		``Vina S'': the binding affinities between the initially generated poses of molecules and the protein pockets; 
		``Vina M'': the binding affinities between the poses after local structure minimization and the protein pockets;
		``Vina D'': the binding affinities between the poses determined by AutoDock Vina~\cite{Eberhardt2021} and the protein pockets;
		``HA'': the percentage of generated molecules with Vina D higher than those of condition molecules;
		``QED'': the drug-likeness score;
		``SA'': the synthesizability score;
		``Div'': the diversity among generated molecules;
		``time'': the time cost to generate molecules.}
\!\! \par
		\par
		\end{footnotesize}
	\end{tablenotes}
\end{threeparttable}
\end{scriptsize}
  \vspace{-10pt}    
\end{table*}


==> tables/docking_results_bond_angles.tex <==
\begin{table*}
	\centering
		\caption{\ziqi{Comparison on Molecule Quality with Shape-Conditioned Molecule Generation Methods}}
	\label{tbl:docking_results_bond_angles}
	\begin{small}
\begin{threeparttable}
	\begin{tabular}{
		@{\hspace{0pt}}l@{\hspace{2pt}}
		@{\hspace{0pt}}c@{\hspace{2pt}}
		%
		@{\hspace{3pt}}c@{\hspace{3pt}}
		%
		@{\hspace{3pt}}c@{\hspace{3pt}}
		@{\hspace{3pt}}c@{\hspace{3pt}}
		@{\hspace{3pt}}c@{\hspace{3pt}}
		@{\hspace{3pt}}c@{\hspace{3pt}}
		@{\hspace{3pt}}c@{\hspace{3pt}}
		@{\hspace{3pt}}c@{\hspace{3pt}}
		@{\hspace{3pt}}c@{\hspace{3pt}}
		%
		%
		}
		\toprule
		Angle & & \AR&  \pockettwomol & \targetdiff & \method & \methodwithsguide &  \methodwithpguide & \methodwithsandpguide \\
		%\multirow{2}{*}{method} & \multirow{2}{*}{\#c\%} &  \multirow{2}{*}{\#u\%} &  \multirow{2}{*}{QED} & \multicolumn{3}{c}{$\nmax=50$} & & \multicolumn{2}{c}{$\nmax=1$}\\
		%\cmidrule(r){5-7} \cmidrule(r){8-10} 
		%& & & & \avgshapesim(std) & \avggraphsim(std  &  \diversity(std  & & \avgshapesim(std) & \avggraphsim(std \\
		\midrule
		CCC & &	0.269& 0.324& 0.253& \textbf{0.225}& 0.258& 0.318& 0.345 \\
		CCO & & 	0.363& 0.356& 0.291& \textbf{0.174}& 0.213& 0.304& 0.322\\
		CNC &  &	0.349& \textbf{0.112}& 0.269& 0.173& 0.201& 0.262& 0.291\\
		OPO &  & 	-& -& -& -& -& -& -\\
		NCC & &	0.310& 0.280& 0.248& \textbf{0.168}& 0.202& 0.289& 0.316\\
		CC=O & & 0.400& 0.200& 0.193& \textbf{0.166}& 0.195& 0.216& 0.245\\
		COC & &	0.378& 0.163& 0.262& \textbf{0.149}& 0.166& 0.238& 0.257\\
		%
		%
		\bottomrule
	\end{tabular}%
	\begin{tablenotes}[normal,flushleft]
		\begin{footnotesize}
	\item 
\!\!Columns represent:  \todo{ziqi: OPO is not common bond pair; need to modify previous scripts in order to calculate OPO.}\par
		\par
		\end{footnotesize}
	\end{tablenotes}
\end{threeparttable}
\end{small}
  \vspace{-10pt}    
\end{table*}


==> tables/docking_results_bond_dist.tex <==
\begin{table*}
	\centering
		\caption{\ziqi{Comparison on Bond Distance Distributions}}
	\label{tbl:docking_results_bond_dist}
	\begin{small}
\begin{threeparttable}
	\begin{tabular}{
		@{\hspace{0pt}}l@{\hspace{2pt}}
		@{\hspace{0pt}}c@{\hspace{2pt}}
		%
		@{\hspace{3pt}}c@{\hspace{3pt}}
		%
		@{\hspace{3pt}}c@{\hspace{3pt}}
		@{\hspace{3pt}}c@{\hspace{3pt}}
		@{\hspace{3pt}}c@{\hspace{3pt}}
		@{\hspace{3pt}}c@{\hspace{3pt}}
		@{\hspace{3pt}}c@{\hspace{3pt}}
		@{\hspace{3pt}}c@{\hspace{3pt}}
		@{\hspace{3pt}}c@{\hspace{3pt}}
		%
		%
		}
		\toprule
		Bond & & \AR&  \pockettwomol & \targetdiff & \method & \methodwithsguide &  \methodwithpguide & \methodwithsandpguide \\
		%\multirow{2}{*}{method} & \multirow{2}{*}{\#c\%} &  \multirow{2}{*}{\#u\%} &  \multirow{2}{*}{QED} & \multicolumn{3}{c}{$\nmax=50$} & & \multicolumn{2}{c}{$\nmax=1$}\\
		%\cmidrule(r){5-7} \cmidrule(r){8-10} 
		%& & & & \avgshapesim(std) & \avggraphsim(std  &  \diversity(std  & & \avgshapesim(std) & \avggraphsim(std \\
		\midrule
		C-C & &	0.499& 0.463& 0.292& \textbf{0.234}& 0.240& 0.313& 0.325 \\
		C=C & & 	0.439& 0.447& 0.378& 0.290& 0.243& 0.189& \textbf{0.182}\\
		C-N &  &	0.247& 0.313& 0.230& 0.218& \textbf{0.216} & 0.247& 0.264\\
		C=N &  & 	0.310& 0.359& 0.139& 0.154& \textbf{0.131}& 0.175& 0.187\\
		C-O & &	0.308& 0.319& 0.289& \textbf{0.226}& 0.228& 0.250& 0.249\\
		C=O & & 	0.439& 0.447& 0.378& 0.290& 0.243& 0.189& \textbf{0.182}\\
		C:C & &	0.377& -& \textbf{0.187} & 0.404& 0.381& 0.259& 0.239\\
		C:N & &	0.385& -& \textbf{0.115} & 0.230& 0.207& 0.161& 0.154\\
		%
		%
		\bottomrule
	\end{tabular}%
	\begin{tablenotes}[normal,flushleft]
		\begin{footnotesize}
	\item 
\!\!Columns represent:  \todo{ziqi: double-check the results of \pockettwomol, their method seems to not generate any aromatic rings.}\par
		\par
		\end{footnotesize}
	\end{tablenotes}
\end{threeparttable}
\end{small}
  \vspace{-10pt}    
\end{table*}


==> tables/docking_results_similarity.tex <==
\begin{table*}[t!]
	\centering
	\caption{{Overall Comparison on Similarity for Pocket-based Molecule Generation}}
	\label{tbl:docking_results_similarity}
	\begin{small}
		\begin{threeparttable}
			\begin{tabular}{
					@{\hspace{0pt}}l@{\hspace{5pt}}
					%
					@{\hspace{3pt}}l@{\hspace{3pt}}
					%
					@{\hspace{3pt}}r@{\hspace{8pt}}
					@{\hspace{3pt}}c@{\hspace{3pt}}
					%
					@{\hspace{3pt}}c@{\hspace{3pt}}
					@{\hspace{3pt}}c@{\hspace{3pt}}
					%
					@{\hspace{0pt}}c@{\hspace{0pt}}
					%
					@{\hspace{3pt}}c@{\hspace{3pt}}
					@{\hspace{3pt}}c@{\hspace{3pt}}
					%
					@{\hspace{3pt}}r@{\hspace{3pt}}
				}
				\toprule
				$\delta_g$  & method          & \#d\%$\uparrow$ & $\diversity_d$$\uparrow$(std) & \avgshapesim$\uparrow$(std) & \avggraphsim$\downarrow$(std) & & \maxshapesim$\uparrow$(std) & \maxgraphsim$\downarrow$(std)       & \#n\%$\uparrow$  \\ 
				\midrule
				%\multirow{6}{0.059\linewidth}{\hspace{0pt}0.1} 
				%& \AR   & 4.4 & 0.781(0.076) & 0.511(0.197) & \textbf{0.056}(0.020) & & 0.619(0.222) & 0.074(0.024) & 21.4  \\
				%& \pockettwomol & 6.6 & 0.795(0.099) & 0.519(0.216) & 0.063(0.020) & & 0.608(0.236) & 0.076(0.022) & \textbf{24.1}  \\
				%& \targetdiff & 2.0 & 0.872(0.041) & 0.619(0.110) & 0.068(0.018) & & 0.721(0.146) & 0.075(0.023) & 17.7  \\
				%& \decompdiffbeta & 0.0 & - & 0.374(0.138) & 0.059(0.031) & & 0.414(0.141) & \textbf{0.058}(0.032) & 9.8  \\
				%& \decompdiffref & 8.5 & 0.805(0.096) & 0.810(0.070) & 0.076(0.018) & & 0.861(0.085) & 0.076(0.020) & 11.3  \\
				%& \methodwithpguide   &  9.9 & \textbf{0.876}(0.041) & 0.795(0.058) & 0.073(0.015) & & 0.869(0.073) & 0.076(0.020) & 17.7  \\
				%& \methodwithsandpguide & \textbf{11.9} & 0.872(0.036) & \textbf{0.813}(0.052) & 0.075(0.014) & & \textbf{0.874}(0.069) & 0.080(0.014) & 17.0  \\
				%\cmidrule{2-10}
				%& improv\% & 40.4$^*$ & 8.8$^*$ & 0.4 & -30.4$^*$ &  & 1.6 & -30.0$^*$ & -26.3$^*$  \\
				%\midrule
				\multirow{7}{0.059\linewidth}{\hspace{0pt}1.0} 
				& \AR & 14.6 & 0.681(0.163) & 0.644(0.119) & 0.236(0.123) & & 0.780(0.110) & 0.284(0.177) & 95.8  \\
				& \pockettwomol & 18.6 & 0.711(0.152) & 0.654(0.131) &   \textbf{0.217}(0.129) & & 0.778(0.121) &   \textbf{0.243}(0.137) &  \textbf{98.3}  \\
				& \targetdiff & 7.1 &  \textbf{0.785}(0.085) & 0.622(0.083) & 0.238(0.122) & & 0.790(0.102) & 0.274(0.158) & 90.4  \\
				%& \decompdiffbeta & 0.1 & 0.589(0.030) & 0.494(0.124) & 0.263(0.143) & & 0.567(0.143) & 0.275(0.162) & 67.7  \\
				& \decompdiffref & 37.3 & 0.721(0.108) & 0.770(0.087) & 0.282(0.130) & & \textbf{0.878}(0.059) & 0.343(0.174) & 83.7  \\
				& \methodwithpguide   &  27.4 & 0.757(0.134) & 0.747(0.078) & 0.265(0.165) & & 0.841(0.081) & 0.272(0.168) & 98.1  \\
				& \methodwithsandpguide &\textbf{45.2} & 0.724(0.142) &   \textbf{0.789}(0.063) & 0.265(0.162) & & 0.876(0.062) & 0.264(0.159) & 97.8  \\
				\cmidrule{2-10}
				& Improv\%  & 21.2$^*$ & -3.6 & 2.5$^*$ & -21.7$^*$ &  & -0.1 & -8.4$^*$ & -0.2  \\
				\midrule
				\multirow{7}{0.059\linewidth}{\hspace{0pt}0.7} 
				& \AR   & 14.5 & 0.692(0.151) & 0.644(0.119) & 0.233(0.116) & & 0.779(0.110) & 0.266(0.140) & 94.9  \\
				& \pockettwomol & 18.6 & 0.711(0.152) & 0.654(0.131) & \textbf{0.217}(0.129) & & 0.778(0.121) & \textbf{0.243}(0.137) & \textbf{98.2}  \\
				& \targetdiff & 7.1 & \textbf{0.786}(0.084) & 0.622(0.083) & 0.238(0.121) & & 0.790(0.101) & 0.270(0.151) & 90.3  \\
				%& \decompdiffbeta & 0.1 & 0.589(0.030) & 0.494(0.124) & 0.263(0.142) & &0.567(0.143) & 0.273(0.156) & 67.6  \\
				& \decompdiffref & 36.2 & 0.721(0.113) & 0.770(0.086) & 0.273(0.123) & & \textbf{0.876}(0.059) & 0.325(0.139) & 82.3  \\
				& \methodwithpguide   &  27.4 & 0.757(0.134) & 0.746(0.078) & 0.263(0.160) & & 0.841(0.081) & 0.271(0.164) & 96.8  \\
				& \methodwithsandpguide      & \textbf{45.0} & 0.732(0.129) & \textbf{0.789}(0.063) & 0.262(0.157) & & \textbf{0.876}(0.063) & 0.262(0.153) & 96.2  \\
				\cmidrule{2-10}
				& Improv\%  & 24.3$^*$ & -3.6 & 2.5$^*$ & -20.8$^*$ &  & 0.0 & -7.6$^*$ & -1.5  \\
				\midrule
				\multirow{7}{0.059\linewidth}{\hspace{0pt}0.5} 
				& \AR   & 14.1 & 0.687(0.160) & 0.639(0.124) & 0.218(0.097) & & 0.778(0.110) & 0.260(0.130) & 89.8  \\
				& \pockettwomol & 18.5 & 0.711(0.152) & 0.649(0.134) & \textbf{0.209}(0.114) & & 0.777(0.121) & \textbf{0.240}(0.131) & \textbf{93.2}  \\
				& \targetdiff & 7.1 & \textbf{0.786}(0.084) & 0.621(0.083) & 0.230(0.111) & & 0.788(0.105) & 0.254(0.127) & 86.5  \\
				%&\decompdiffbeta & 0.1 & 0.595(0.025) & 0.494(0.124) & 0.254(0.129) & & 0.565(0.142) & 0.259(0.138) & 63.9  \\
				& \decompdiffref & 34.7 & 0.730(0.105) & 0.769(0.086) & 0.261(0.109) & & 0.874(0.080) & 0.301(0.117) & 77.3   \\
				& \methodwithpguide  &  27.2 & 0.765(0.123) & 0.749(0.075) & 0.245(0.135) & & 0.840(0.082) & 0.252(0.137) & 88.6  \\
				& \methodwithsandpguide & \textbf{44.3} & 0.738(0.122) & \textbf{0.791}(0.059) & 0.247(0.132) &  & \textbf{0.875}(0.065) & 0.249(0.130) & 88.8  \\
				\cmidrule{2-10}
				& Improv\%   & 27.8$^*$ & -2.7 & 2.9$^*$ & -17.6$^*$ &  & 0.2 & -3.4 & -4.7$^*$  \\
				\midrule
				\multirow{7}{0.059\linewidth}{\hspace{0pt}0.3} 
				& \AR   & 12.2 & 0.704(0.146) & 0.614(0.146) & 0.164(0.059) & & 0.751(0.138) & 0.206(0.059) & 66.4  \\
				& \pockettwomol & 17.1 & 0.731(0.129) & 0.617(0.163) & \textbf{0.155}(0.056) & & 0.740(0.159) & \textbf{0.190}(0.076) & \textbf{71.0}  \\
				& \targetdiff & 6.2 & \textbf{0.809}(0.061) & 0.619(0.087) & 0.181(0.068) & & 0.768(0.119) & 0.196(0.076) & 61.7  \\				
                %& \decompdiffbeta & 0.0 & - & 0.489(0.124) & 0.195(0.080) & & 0.547(0.139) & 0.203(0.087) & 42.0  \\
				& \decompdiffref & 27.7 & 0.775(0.081) & 0.767(0.086) & 0.202(0.062) & & 0.854(0.093) & 0.216(0.068) & 52.6  \\
				& \methodwithpguide   &  24.4 & 0.805(0.084) & 0.763(0.066) & 0.180(0.074) & & 0.847(0.080) & \textbf{0.190}(0.059) & 61.4  \\
				& \methodwithsandpguide & \textbf{36.3} & 0.789(0.081) & \textbf{0.800}(0.056) & 0.181(0.071) & &\textbf{0.878}(0.067) & \textbf{0.190}(0.078) & 61.8  \\
				\cmidrule{2-10}
				& improv\% & 31.1$^*$ & 3.9$^*$ & 4.3$^*$ & -16.5$^*$ &  & 2.8$^*$ & 0.0 & -12.9$^*$  \\
				\bottomrule
			\end{tabular}%
			\begin{tablenotes}[normal,flushleft]
				\begin{footnotesize}
					\item 
					\!\!Columns represent: \ziqi{``$\delta_g$'': the graph similarity constraint; ``\#n\%'': the percentage of molecules that satisfy the graph similarity constraint ($\graphsim<=\delta_g$);
						``\#d\%'': the percentage of molecules that satisfy the graph similarity constraint and are with high \shapesim ($\shapesim>=0.8$);
						``\avgshapesim/\avggraphsim'': the average of shape or graph similarities between the condition molecules and generated molecules with $\graphsim<=\delta_g$;
						``\maxshapesim'': the maximum of shape similarities between the condition molecules and generated molecules with $\graphsim<=\delta_g$;
						``\maxgraphsim'': the graph similarities between the condition molecules and the molecules with the maximum shape similarities and $\graphsim<=\delta_g$;
						``\diversity'': the diversity among the generated molecules.
						%
						``$\uparrow$'' represents higher values are better, and ``$\downarrow$'' represents lower values are better.
						%
						Best values are in \textbf{bold}, and second-best values are \underline{underlined}. 
					} 
					%\todo{double-check the significance value}
					\par
					\par
				\end{footnotesize}
			\end{tablenotes}
		\end{threeparttable}
	\end{small}
	\vspace{-10pt}    
\end{table*}

==> tables/overall_docking_results_quality0.1.tex <==
\begin{table*}
	\centering
		\caption{\ziqi{Comparison on Molecule Quality with Pocket-based Molecule Generation Methods with Pocket Known ($\delta_g$=0.1)}}
	\label{tbl:overall_docking_results_quality_01}
	\begin{small}
\begin{threeparttable}
	\begin{tabular}{
		@{\hspace{0pt}}l@{\hspace{14pt}}
		@{\hspace{0pt}}l@{\hspace{2pt}}
		%
		@{\hspace{4pt}}c@{\hspace{4pt}}
		%
		@{\hspace{3pt}}c@{\hspace{3pt}}
		@{\hspace{3pt}}c@{\hspace{3pt}}
		@{\hspace{3pt}}c@{\hspace{3pt}}
		@{\hspace{3pt}}c@{\hspace{3pt}}
		@{\hspace{3pt}}c@{\hspace{3pt}}
		@{\hspace{3pt}}c@{\hspace{3pt}}
		@{\hspace{3pt}}c@{\hspace{3pt}}
		%
		%
		}
		\toprule
		group & metric & & \AR & \pockettwomol & \targetdiff & \decompdiffbeta & \decompdiffref & \methodwithpguide & \methodwithsandpguide \\
		%\multirow{2}{*}{method} & \multirow{2}{*}{\#c\%} &  \multirow{2}{*}{\#u\%} &  \multirow{2}{*}{QED} & \multicolumn{3}{c}{$\nmax=50$} & & \multicolumn{2}{c}{$\nmax=1$}\\
		%\cmidrule(r){5-7} \cmidrule(r){8-10} 
		%& & & & \avgshapesim(std) & \avggraphsim(std  &  \diversity(std  & & \avgshapesim(std) & \avggraphsim(std \\
		\midrule
		\multirow{2}{*}{stability} 
		& atom stability ($\uparrow$) & 
			& 0.941 & 0.856 & \textbf{0.953} & 0.887 & 0.938 & 0.943 & 0.942     \\
		& molecule stability ($\uparrow$) & 
			& \textbf{0.700} & 0.264 & 0.577 & 0.143 & 0.564 & 0.691 & 0.652     \\
		\midrule
		\multirow{3}{*}{Drug-likeness}
& QED ($\uparrow$) & & 0.530 & 0.590 & 0.468 & 0.387 & 0.445 & \textbf{0.616} & 0.609    \\
& SA ($\uparrow$) & & 0.644 & \textbf{0.738} & 0.579 & 0.566 & 0.660 & 0.652 & 0.636    \\
& Lipinski ($\uparrow$) & & 4.869 & \textbf{4.898} & 4.560 & 3.916 & 4.216 & 4.854 & 4.818    \\
		\midrule
		\multirow{4}{*}{3D structures} 
& RMSD ($\downarrow$) & & 0.730 & \textbf{0.455} & 1.066 & 1.465 & 0.884 & 0.716 & 0.756    \\
& JS. bond lengths ($\downarrow$) & & 0.567 & 0.549 & 0.502 & 0.472 & 0.462 & \textbf{0.406} & 0.439    \\
& JS. bond angles ($\downarrow$) & & 0.332 & 0.531 & 0.383 & \textbf{0.269} & 0.301 & 0.309 & 0.333    \\
& JS. dihedral angles ($\downarrow$) & & 0.458 & 0.320 & 0.317 & 0.322 & 0.286 & \textbf{0.230} & 0.232    \\
		\midrule
		\multirow{5}{*}{Bonds} 
& JS. \#bonds per atoms ($\downarrow$) & & 0.475 & 0.437 & 0.254 & \textbf{0.174} & 0.440 & 0.429 & 0.457    \\
& JS. basic bond types ($\downarrow$) & & 0.300 & 0.465 & 0.281 & \textbf{0.199} & 0.236 & 0.247 & 0.264    \\
& JS. freq. bond types ($\downarrow$) & & 0.325 & 0.524 & 0.350 & \textbf{0.231} & 0.246 & 0.309 & 0.324    \\
& JS. freq. bond pairs ($\downarrow$) & & 0.332 & 0.531 & 0.383 & \textbf{0.269} & 0.301 & 0.309 & 0.333    \\
& JS. freq. bond triplets ($\downarrow$) & & 0.340 & 0.610 & 0.400 & \textbf{0.298} & 0.321 & 0.341 & 0.366    \\
		\midrule
		\multirow{3}{*}{Rings} 
& JS. \#rings ($\downarrow$) & & 0.401 & 0.344 & \textbf{0.222} & 0.335 & 0.320 & 0.406 & 0.424    \\
& JS. \#n-sized rings ($\downarrow$) & & 0.176 & \textbf{0.110} & 0.162 & 0.208 & 0.162 & 0.169 & 0.185    \\
& \#Intersecting rings ($\uparrow$) & & 5 & 2 & 5 & 5 & \textbf{6} & 5 & 5    \\
		%
		%
		\bottomrule
	\end{tabular}%
	\begin{tablenotes}[normal,flushleft]
		\begin{footnotesize}
	\item 
\!\!Columns represent:  \todo{ziqi: the calculation of RMSD metric is a little bit time-consuming, as it requires the optimization of the force field. I will update the results later.}\par
		\par
		\end{footnotesize}
	\end{tablenotes}
\end{threeparttable}
\end{small}
  \vspace{-10pt}    
\end{table*}


==> tables/overall_docking_results_quality0.3.tex <==
\begin{table*}
	\centering
		\caption{\ziqi{Comparison on Molecule Quality with Pocket-based Molecule Generation Methods with Pocket Known ($\delta_g$=0.3)}}
	\label{tbl:overall_docking_results_quality_03}
	\begin{small}
\begin{threeparttable}
	\begin{tabular}{
		@{\hspace{0pt}}l@{\hspace{14pt}}
		@{\hspace{0pt}}l@{\hspace{2pt}}
		%
		@{\hspace{4pt}}c@{\hspace{4pt}}
		%
		%@{\hspace{3pt}}c@{\hspace{3pt}}
		@{\hspace{3pt}}c@{\hspace{3pt}}
		@{\hspace{3pt}}c@{\hspace{3pt}}
		@{\hspace{3pt}}c@{\hspace{3pt}}
		@{\hspace{3pt}}c@{\hspace{3pt}}
		@{\hspace{3pt}}c@{\hspace{3pt}}
		@{\hspace{3pt}}c@{\hspace{3pt}}
		%
		%
		}
		\toprule
		group & metric & & \AR & \pockettwomol & \targetdiff & \decompdiffref & \methodwithpguide & \methodwithsandpguide \\
		%\multirow{2}{*}{method} & \multirow{2}{*}{\#c\%} &  \multirow{2}{*}{\#u\%} &  \multirow{2}{*}{QED} & \multicolumn{3}{c}{$\nmax=50$} & & \multicolumn{2}{c}{$\nmax=1$}\\
		%\cmidrule(r){5-7} \cmidrule(r){8-10} 
		%& & & & \avgshapesim(std) & \avggraphsim(std  &  \diversity(std  & & \avgshapesim(std) & \avggraphsim(std \\
		\midrule
		\multirow{2}{*}{stability} 
		& atom stability ($\uparrow$) & 
			& 0.926 & 0.845 & \textbf{0.951} & 0.923 & 0.936 & 0.914     \\
		& molecule stability ($\uparrow$) & 
			& 0.556 & 0.183 & 0.471 & 0.410 & \textbf{0.587} & 0.514     \\
		\midrule
		\multirow{3}{*}{Drug-likeness}
& QED ($\uparrow$) & & 0.507 & 0.579 & 0.471 & 0.490 & \textbf{0.645} & 0.635    \\
& SA ($\uparrow$) & & 0.655 & \textbf{0.757} & 0.582 & 0.655 & 0.625 & 0.615    \\
& Lipinski ($\uparrow$) & & 4.761 & \textbf{4.903} & 4.482 & 4.477 & 4.865 & 4.856    \\
		\midrule
		\multirow{4}{*}{3D structures} 
& RMSD ($\downarrow$) & & 0.732 & \textbf{0.441} & 1.030 & 0.925 & 0.781 & 0.811    \\
& JS. bond lengths ($\downarrow$) & & 0.567 & 0.549 & 0.502 & 0.462 & \textbf{0.406} & 0.439    \\
& JS. bond angles ($\downarrow$) & & 0.332 & 0.531 & 0.383 & 0.301 & 0.309 & 0.333    \\
& JS. dihedral angles ($\downarrow$) & & 0.458 & 0.320 & 0.317 & 0.286 & \textbf{0.230} & 0.232    \\
		\midrule
		\multirow{5}{*}{Bonds} 
& JS. \#bonds per atoms ($\downarrow$) & & 0.466 & 0.425 & 0.307 & 0.318 & 0.380 & 0.392    \\
& JS. basic bond types ($\downarrow$) & & 0.265 & 0.465 & 0.291 & 0.217 & 0.255 & 0.267    \\
& JS. freq. bond types ($\downarrow$) & & 0.325 & 0.524 & 0.350 & 0.246 & 0.309 & 0.324    \\
& JS. freq. bond pairs ($\downarrow$) & & 0.332 & 0.531 & 0.383 & 0.301 & 0.309 & 0.333    \\
& JS. freq. bond triplets ($\downarrow$) & & 0.340 & 0.610 & 0.400 & 0.321 & 0.341 & 0.366    \\
		\midrule
		\multirow{3}{*}{Rings} 
& JS. \#rings ($\downarrow$) & & 0.387 & 0.334 & \textbf{0.291} & 0.292 & 0.350 & 0.354    \\
& JS. \#n-sized rings ($\downarrow$) & & 0.167 & \textbf{0.101} & 0.171 & 0.166 & 0.178 & 0.184    \\
& \#Intersecting rings ($\uparrow$) & & 5 & 2 & 5 & \textbf{6} & 5 & 5    \\
		%
		%
		\bottomrule
	\end{tabular}%
	\begin{tablenotes}[normal,flushleft]
		\begin{footnotesize}
	\item 
\!\!Columns represent:  \todo{ziqi: the calculation of RMSD metric is a little bit time-consuming, as it requires the optimization of the force field. I will update the results later.}\par
		\par
		\end{footnotesize}
	\end{tablenotes}
\end{threeparttable}
\end{small}
  \vspace{-10pt}    
\end{table*}


==> tables/overall_docking_results_quality0.5.tex <==
\begin{table*}
	\centering
		\caption{\ziqi{Comparison on Molecule Quality with Pocket-based Molecule Generation Methods with Pocket Known ($\delta_g$=0.5)}}
	\label{tbl:overall_docking_results_quality_05}
	\begin{small}
\begin{threeparttable}
	\begin{tabular}{
		@{\hspace{0pt}}l@{\hspace{14pt}}
		@{\hspace{0pt}}l@{\hspace{2pt}}
		%
		@{\hspace{4pt}}c@{\hspace{4pt}}
		%
		%@{\hspace{3pt}}c@{\hspace{3pt}}
		@{\hspace{3pt}}c@{\hspace{3pt}}
		@{\hspace{3pt}}c@{\hspace{3pt}}
		@{\hspace{3pt}}c@{\hspace{3pt}}
		@{\hspace{3pt}}c@{\hspace{3pt}}
		@{\hspace{3pt}}c@{\hspace{3pt}}
		@{\hspace{3pt}}c@{\hspace{3pt}}
		%
		%
		}
		\toprule
		group & metric & & \AR & \pockettwomol & \targetdiff & \decompdiffref & \methodwithpguide & \methodwithsandpguide \\
		%\multirow{2}{*}{method} & \multirow{2}{*}{\#c\%} &  \multirow{2}{*}{\#u\%} &  \multirow{2}{*}{QED} & \multicolumn{3}{c}{$\nmax=50$} & & \multicolumn{2}{c}{$\nmax=1$}\\
		%\cmidrule(r){5-7} \cmidrule(r){8-10} 
		%& & & & \avgshapesim(std) & \avggraphsim(std  &  \diversity(std  & & \avgshapesim(std) & \avggraphsim(std \\
		\midrule
		\multirow{2}{*}{stability} 
		& atom stability ($\uparrow$) & 
			& 0.914 & 0.840 & \textbf{0.950} & 0.916 & 0.916 & 0.895     \\
		& molecule stability ($\uparrow$) & 
			& 0.487 & 0.146 & 0.428 & 0.344 & \textbf{0.489} & 0.417     \\
		\midrule
		\multirow{3}{*}{Drug-likeness}
		& QED ($\uparrow$) & & 0.512 & 0.574 & 0.478 & 0.504 & \textbf{0.643} & 0.633    \\
		& SA ($\uparrow$) & & 0.655 & \textbf{0.755} & 0.583 & 0.661 & 0.624 & 0.616    \\
		& Lipinski ($\uparrow$) & & 4.763 & \textbf{4.895} & 4.513 & 4.501 & 4.844 & 4.832    \\
		\midrule
		\multirow{4}{*}{3D structures} 
		& RMSD ($\downarrow$) & & 0.734 & \textbf{0.455} & 1.023 & 0.921 & 0.777 & 0.802    \\
		& JS. bond lengths ($\downarrow$) & & 0.567 & 0.549 & 0.502 & 0.462 & \textbf{0.406} & 0.439    \\
		& JS. bond angles ($\downarrow$) & & 0.332 & 0.531 & 0.383 & 0.301 & 0.309 & 0.333    \\
		& JS. dihedral angles ($\downarrow$) & & 0.458 & 0.320 & 0.317 & 0.286 & \textbf{0.230} & 0.232    \\
		\midrule
		\multirow{5}{*}{Bonds}
		& JS. \#bonds per atoms ($\downarrow$) & & {0.469} & 0.429 & 0.308 & 0.335 & 0.391 & 0.399    \\
		& JS. basic bond types ($\downarrow$) & & 0.258 & {0.465} & 0.289 & 0.216 & 0.253 & 0.266    \\
		& JS. freq. bond types ($\downarrow$) & & 0.325 & {0.524} & 0.350 & 0.246 & 0.309 & 0.324    \\
		& JS. freq. bond pairs ($\downarrow$) & & 0.332 & 0.531 & 0.383 & 0.301 & 0.309 & 0.333    \\
		& JS. freq. bond triplets ($\downarrow$) & & 0.340 & {0.610} & 0.400 & 0.321 & 0.341 & 0.366    \\
		\midrule
		\multirow{3}{*}{Rings} 
		& JS. \#rings ($\downarrow$) & & {0.377} & 0.346 & \textbf{0.289} & 0.294 & 0.360 & 0.361    \\
		& JS. \#n-sized rings ($\downarrow$) & & 0.166 & \textbf{0.104} & 0.172 & 0.163 & 0.183 & 0.189    \\
		& \#Intersecting rings ($\uparrow$) & & 5 & 2 & 5 & \textbf{6} & 5 & 5    \\
		%
		\bottomrule
	\end{tabular}%
	\begin{tablenotes}[normal,flushleft]
		\begin{footnotesize}
	\item 
\!\!Columns represent:  \todo{ziqi: the calculation of RMSD metric is a little bit time-consuming, as it requires the optimization of the force field. I will update the results later.}\par
		\par
		\end{footnotesize}
	\end{tablenotes}
\end{threeparttable}
\end{small}
  \vspace{-10pt}    
\end{table*}


==> tables/overall_docking_results_quality0.7.tex <==
\begin{table*}
	\centering
		\caption{\ziqi{Comparison on Molecule Quality with Pocket-based Molecule Generation Methods with Pocket Known ($\delta_g$=0.7)}}
	\label{tbl:overall_docking_results_quality_07}
	\begin{small}
\begin{threeparttable}
	\begin{tabular}{
		@{\hspace{0pt}}l@{\hspace{14pt}}
		@{\hspace{0pt}}l@{\hspace{2pt}}
		%
		@{\hspace{4pt}}c@{\hspace{4pt}}
		%
		%@{\hspace{3pt}}c@{\hspace{3pt}}
		@{\hspace{3pt}}c@{\hspace{3pt}}
		@{\hspace{3pt}}c@{\hspace{3pt}}
		@{\hspace{3pt}}c@{\hspace{3pt}}
		@{\hspace{3pt}}c@{\hspace{3pt}}
		@{\hspace{3pt}}c@{\hspace{3pt}}
		@{\hspace{3pt}}c@{\hspace{3pt}}
		%
		%
		}
		\toprule
		group & metric & & \AR & \pockettwomol & \targetdiff & \decompdiffref & \methodwithpguide & \methodwithsandpguide \\
		%\multirow{2}{*}{method} & \multirow{2}{*}{\#c\%} &  \multirow{2}{*}{\#u\%} &  \multirow{2}{*}{QED} & \multicolumn{3}{c}{$\nmax=50$} & & \multicolumn{2}{c}{$\nmax=1$}\\
		%\cmidrule(r){5-7} \cmidrule(r){8-10} 
		%& & & & \avgshapesim(std) & \avggraphsim(std  &  \diversity(std  & & \avgshapesim(std) & \avggraphsim(std \\
		\midrule
		\multirow{2}{*}{stability} 
		& atom stability ($\uparrow$) & &
			0.911 & 0.837 & \textbf{0.949} & 0.914 & 0.901 & 0.880     \\
		& molecule stability ($\uparrow$) & &
			\textbf{0.469} & 0.139 & 0.420 & 0.331 & 0.456 & 0.390     \\
		\midrule
		\multirow{3}{*}{Drug-likeness}
		& QED ($\uparrow$) & & 0.513 & 0.573 & 0.480 & 0.501 & \textbf{0.640} & 0.630    \\
		& SA ($\uparrow$) & & 0.656 & \textbf{0.756} & 0.585 & {0.661} & 0.619 & 0.611    \\
		& Lipinski ($\uparrow$) & & 4.763 & \textbf{4.899} & 4.522 & 4.484 & 4.819 & 4.801    \\
		\midrule
		\multirow{4}{*}{3D structures} 
		& RMSD ($\downarrow$) & & 0.730 & \textbf{0.451} & 1.015 & 0.920 & 0.783 & 0.809    \\
		& JS. bond lengths ($\downarrow$) & & 0.567 & 0.549 & 0.502 & 0.462 & \textbf{0.406} & 0.439    \\
		& JS. bond angles ($\downarrow$) & & 0.332 & 0.531 & 0.383 & 0.301 & 0.309 & 0.333    \\
		& JS. dihedral angles ($\downarrow$) & & 0.458 & 0.320 & 0.317 & 0.286 & \textbf{0.230} & 0.232    \\
		\midrule
		\multirow{5}{*}{Bonds} 
		& JS. \#bonds per atoms ($\downarrow$) & & 0.469 & 0.433 & 0.311 & 0.336 & 0.391 & 0.399    \\
		& JS. basic bond types ($\downarrow$) & & 0.259 & 0.465 & 0.290 & 0.217 & 0.253 & 0.268    \\
		& JS. freq. bond types ($\downarrow$) & & 0.325 & 0.524 & 0.350 & 0.246 & 0.309 & 0.324    \\
		& JS. freq. bond pairs ($\downarrow$) & & 0.332 & 0.531 & 0.383 & 0.301 & 0.309 & 0.333    \\
		& JS. freq. bond triplets ($\downarrow$) & & 0.340 & 0.610 & 0.400 & 0.321 & 0.341 & 0.366    \\
		\midrule
		\multirow{3}{*}{Rings} 
		& JS. \#rings ($\downarrow$) & & 0.376 & 0.352 & \textbf{0.293} & 0.294 & 0.360 & 0.360    \\
		& JS. \#n-sized rings ($\downarrow$) & & 0.165 & \textbf{0.105} & 0.173 & 0.163 & 0.187 & 0.194    \\
		& \#Intersecting rings ($\uparrow$) & & 5 & 2 & 5 & \textbf{6} & 5 & 5    \\
		%
		%
		\bottomrule
	\end{tabular}%
	\begin{tablenotes}[normal,flushleft]
		\begin{footnotesize}
	\item 
\!\!Columns represent:  \todo{ziqi: the calculation of RMSD metric is a little bit time-consuming, as it requires the optimization of the force field. I will update the results later.}\par
		\par
		\end{footnotesize}
	\end{tablenotes}
\end{threeparttable}
\end{small}
  \vspace{-10pt}    
\end{table*}


==> tables/overall_results.tex <==
\begin{table*}
	\centering
		\caption{{Overall Comparison on Shape-Conditioned Molecule Generation (old table)}}
	\label{tbl:overall}
	\begin{small}
\begin{threeparttable}
	\begin{tabular}{
		@{\hspace{0pt}}l@{\hspace{2pt}}
		%
		@{\hspace{5pt}}r@{\hspace{5pt}}
		@{\hspace{5pt}}r@{\hspace{5pt}}
		@{\hspace{5pt}}r@{\hspace{5pt}}
		@{\hspace{5pt}}r@{\hspace{5pt}}
		%
		%
		@{\hspace{5pt}}r@{\hspace{5pt}}
		%
		@{\hspace{5pt}}r@{\hspace{5pt}}
		%
		@{\hspace{0pt}}c@{\hspace{0pt}}
		%
	    	@{\hspace{5pt}}c@{\hspace{5pt}}
		%
		@{\hspace{5pt}}c@{\hspace{5pt}}
		%
		@{\hspace{5pt}}c@{\hspace{3pt}}
		%
		}
		\toprule
		method & \#v\% & \#s\% & \#u\%  & \qed  & \avgshapesim(std) & \avggraphsim(std) & & \maxshapesim(std) & \maxgraphsim(std) &  \diversity(std) \\
		%\multirow{2}{*}{method} & \multirow{2}{*}{\#c\%} &  \multirow{2}{*}{\#u\%} &  \multirow{2}{*}{QED} & \multicolumn{3}{c}{$\nmax=50$} & & \multicolumn{2}{c}{$\nmax=1$}\\
		%\cmidrule(r){5-7} \cmidrule(r){8-10} 
		%& & & & \avgshapesim(std) & \avggraphsim(std  &  \diversity(std  & & \avgshapesim(std) & \avggraphsim(std \\
		\midrule
		\dataset                              & 100.0  & 100.0 & 100.0 & 0.795 & 0.729 (0.039) & 0.226 (0.038) & & 0.807 (0.042) & 0.241 (0.087) & 0.759 (0.015)\\
		\squid ($\lambda$=0.3)      & 100.0  & 100.0 &   94.2 & 0.766 & 0.717 (0.083) & 0.349 (0.088) & & 0.904 (0.070) & 0.549 (0.243) & 0.677 (0.065) \\
		\squid ($\lambda$=1.0)      & 100.0  & 100.0 &   95.0 & 0.760 & 0.670 (0.069) & 0.235 (0.045) & & 0.842 (0.061) & 0.271 (0.096) & 0.744 (0.046) \\
		\method                              & 99.6 & 98.8 & 100.0 & 0.748 & 0.689 (0.044) & 0.239 (0.049) & & 0.803 (0.042) & 0.243 (0.068) & 0.712 (0.055) \\
		\methodwithguide               & 99.6 & 98.7 & 100.0 & 0.749 & 0.746 (0.036) & 0.241 (0.050) & & 0.852 (0.034) & 0.247 (0.068) & 0.703 (0.053) \\
		%\methodwithguide                 & 96.8\% & 100.0\% & 0.630 & 0.794 (0.034 & 0.236 (0.051 & 0.703 (0.053 & & 0.890 (0.029 & 0.244 (0.067\\
		%
		\bottomrule
	\end{tabular}%
	\begin{tablenotes}[normal,flushleft]
		\begin{footnotesize}
	\item 
\!\!Columns represent: \ziqi{``\#v\%'': the percentage of valid molecules; ``\#s\%'': the percentage of valid and connected molecules;}%``\#c\%": the percentage of connected molecules; 
``\#u\%'': the percentage of unique molecules;
``\qed'': the average drug-likeness of generated molecules;
``\avgshapesim/\avggraphsim'': the average of shape or graph similarities between the condition molecules and generated molecules; ``std": the standard deviation;
``\maxshapesim'': the maximum of shape similarities between the condition molecules and generated molecules;
``\maxgraphsim'': the graph similarities between the condition molecules and the molecules with the maximum shape similarities;
``\diversity'': the diversity among the generated molecules. \par
		\par
		\end{footnotesize}
	\end{tablenotes}
\end{threeparttable}
\end{small}
  \vspace{-10pt}    
\end{table*}


==> tables/overall_results_docking.tex <==
\begin{table*}[h!]
	\centering
		\caption{\ziqi{Overall Comparison on Pocket-based Molecule Generation}}
	\label{tbl:overall_results_docking}
	\begin{small}
\begin{threeparttable}
	\begin{tabular}{
		@{\hspace{4pt}}l@{\hspace{4pt}}
		%
		@{\hspace{4pt}}l@{\hspace{4pt}}
		%
		@{\hspace{4pt}}r@{\hspace{4pt}}
		@{\hspace{4pt}}r@{\hspace{4pt}}
		@{\hspace{4pt}}r@{\hspace{4pt}}
		%
		@{\hspace{5pt}}r@{\hspace{5pt}}
		%
		@{\hspace{4pt}}r@{\hspace{4pt}}
		@{\hspace{4pt}}r@{\hspace{4pt}}
		%
		@{\hspace{5pt}}r@{\hspace{5pt}}
		%
		@{\hspace{4pt}}r@{\hspace{4pt}}
		@{\hspace{4pt}}r@{\hspace{4pt}}
		%
		%@{\hspace{5pt}}r@{\hspace{5pt}}
		%
		%@{\hspace{2pt}}r@{\hspace{2pt}}
	    %@{\hspace{2pt}}r@{\hspace{2pt}}
		%
		@{\hspace{5pt}}r@{\hspace{5pt}}
		%
		@{\hspace{2pt}}r@{\hspace{2pt}}
		@{\hspace{2pt}}r@{\hspace{2pt}}
		%
		@{\hspace{5pt}}r@{\hspace{5pt}}
		%
		@{\hspace{2pt}}r@{\hspace{2pt}}
		@{\hspace{2pt}}r@{\hspace{2pt}}
		%
		@{\hspace{5pt}}r@{\hspace{5pt}}
		%
		@{\hspace{2pt}}r@{\hspace{2pt}}
		@{\hspace{2pt}}r@{\hspace{2pt}}
		%
		%@{\hspace{5pt}}r@{\hspace{5pt}}
		%
		%@{\hspace{2pt}}r@{\hspace{2pt}}
		}
		\toprule
		\multirow{2}{*}{type} & \multirow{2}{*}{method} & \multirow{2}{*}{\#v\%} & \multicolumn{2}{c}{Vina S$\downarrow$} & & \multicolumn{2}{c}{Vina M$\downarrow$} & & \multicolumn{2}{c}{Vina D$\downarrow$} 
        %& & \multicolumn{2}{c}{HA\%$\uparrow$}  
        & & \multicolumn{2}{c}{QED$\uparrow$} 
        & & \multicolumn{2}{c}{SA$\uparrow$} 
        & & \multicolumn{2}{c}{Div$\uparrow$} \\ 
        %& & \multirow{2}{*}{SR\%$\uparrow$} \\
	    \cmidrule{4-5}\cmidrule{7-8} \cmidrule{10-11} \cmidrule{13-14} \cmidrule{16-17} \cmidrule{19-20}
		& & & Avg. & Med. 
        & & Avg. & Med. 
        & & Avg. & Med. 
        %& & Avg. & Med.  
        & & Avg. & Med.  
        & & Avg. & Med.  
        & & Avg. & Med.  \\
        %& & \\
		%\multirow{2}{*}{method} & \multirow{2}{*}{\#c\%} &  \multirow{2}{*}{\#u\%} &  \multirow{2}{*}{QED} & \multicolumn{3}{c}{$\nmax=50$} & & \multicolumn{2}{c}{$\nmax=1$}\\
		%\cmidrule(r){5-7} \cmidrule(r){8-10} 
		%& & & & \avgshapesim(std) & \avggraphsim(std  &  \diversity(std  & & \avgshapesim(std) & \avggraphsim(std \\
		\midrule
		- & Reference & - & -6.36 & -6.46 & & -6.71 & -6.49 & & -7.45 & -7.26 & 
        %& - & - & 
        & 0.48 & 0.47 & & 0.73 & 0.74 & & - & - \\
        %&& & 25.0 \\
		\midrule
		\multirow{6}{*}{PM} 
		& \ligan                             & - & - & - & & - & - & & -6.33 & -6.20 
        %& & 21.1 & 11.1 
        & & 0.39 & 0.39 & & 0.59 & 0.56 & & 0.66 & 0.67\\ %& & 3.9 \\
		& \graphbp                           & - & - & - & & - & - & & -4.80 & -4.70 
        %& & 14.2 & 6.7 
        & & 0.43 & 0.45 & & 0.49 & 0.48 & & \textbf{0.79} & \textbf{0.78}\\ 
        %& & 0.1 \\
		& \AR & 92.95 & \textbf{-5.75} & \underline{-5.64} & & -6.18 & -5.88 & & -6.75 & -6.62 
        %& & 37.9 & 31.0 
        & & 0.51 & 0.50 & & 0.63 & 0.63 & & 0.70 & 0.70\\ %& & 7.1 \\
		& \pockettwomol                      & \textbf{98.31} & -5.14 & -4.70 & & -6.42 & -5.82 & & -7.15 & -6.79 
        %& & 48.4 & 51.0 
        & & \underline{0.56} & \underline{0.57} & & \textbf{0.74} & \textbf{0.75} & & 0.69 & 0.71\\ 
        %& & \textbf{24.4} \\
		& \targetdiff & 90.36 & -5.47 & \textbf{-6.30} & & \textbf{-6.64} & \textbf{-6.83} & & \textbf{-7.80} & \textbf{-7.91} 
        %& & 58.1 & 59.1 
        & & 0.48 & 0.48 & & 0.58 & 0.58 & & \underline{0.72} & 0.71\\ %& & 10.5 \\
		%& \decompdiffbeta                    & 63.03 & -5.38 & -6.16 & & \textbf{-7.17} & \textbf{-7.32} & & \textbf{-8.81} & \textbf{-8.77} & & \textbf{72.2} & \textbf{89.1} & & 0.38 & 0.35 & & 0.57 & 0.57 & & 0.59 & 0.59 & & 16.6 \\ 
		& \decompdiffref & 83.72 & -5.16 & -5.26 & & -6.03 & -6.00 & & -7.01 & -7.16 
        %& & 47.8 & 48.7 
        & & 0.50 & 0.50 & & \underline{0.66} & \underline{0.65} & & \underline{0.72} & \underline{0.72}\\ %& & 15.1 \\
		%\midrule
		%\multirow{2}{*}{PU} 
		%& \method                           & 98.31 & 17.96 & 12.56 & & -1.73 & -3.93 & & -6.85 & -7.04 & & 42.4 & 40.4 & & \textbf{0.66} & \textbf{0.68} & & 0.68 & 0.68 & & 0.72 & 0.74 & & 16.8 \\
		%& \methodwithsguide          & 98.18 & 1.13 & -0.18 & & -4.63 & -4.72 & & -6.92 & -7.19 & & 46.2 & 44.0 & & \textbf{0.66} & 0.67 & & 0.67 & 0.67 & & 0.71 & 0.73 & & 16.7 \\
		\midrule
		\multirow{2}{*}{PG}
		& \methodwithpguide & \underline{98.14} & -5.36 & -5.48 & & -6.52 & -6.17 & & \underline{-7.61} & \underline{-7.64} 
        %& & 58.8 & 57.6 
        & & \textbf{0.64} & \textbf{0.66} & & 0.62 & 0.63 & & 0.67 & 0.70 \\
        %& & 13.7 \\
		& \methodwithsandpguide   & 97.84 & \underline{-5.66} & -5.61 & & \underline{-6.61} & \underline{-6.21} & & -7.58 & -7.59 
        %& & 57.6 & 58.4 
        & & 0.63 & 0.65 & & 0.61 & 0.62 & & 0.67 & 0.67\\ %& & 12.2 \\
		\bottomrule
	\end{tabular}%
	\begin{tablenotes}[normal,flushleft]
		\begin{footnotesize}
	\item 
\!\!Columns represent: \todo{\textbf{from Ziqi}: (1) considering whether to add the time cost for inference into the table; our model is much more efficient than our baselines as it does not explicitly model the protein pocket; (2) results need to be updated. all the baselines generate 100 molecules for each protein, while our method only generates 50 molecules. new docking results will be available today. }\par
		\par
		\end{footnotesize}
	\end{tablenotes}
\end{threeparttable}
\end{small}
  \vspace{-10pt}    
\end{table*}


==> tables/overall_results_docking2.tex <==
\begin{table*}[!ht]
	\centering
		\caption{\ziqi{Overall Comparison on Pocket-based Molecule Generation}}
	\label{tbl:overall_results_docking2}
\begin{threeparttable}
	\begin{scriptsize}
	\begin{tabular}{
		@{\hspace{2pt}}l@{\hspace{2pt}}
		%
		@{\hspace{2pt}}l@{\hspace{2pt}}
		%
		@{\hspace{2pt}}r@{\hspace{2pt}}
		@{\hspace{2pt}}r@{\hspace{2pt}}
		%
		@{\hspace{4pt}}r@{\hspace{4pt}}
		%
		@{\hspace{2pt}}r@{\hspace{2pt}}
		@{\hspace{2pt}}r@{\hspace{2pt}}
		%
		@{\hspace{5pt}}r@{\hspace{5pt}}
		%
		@{\hspace{2pt}}r@{\hspace{2pt}}
		@{\hspace{2pt}}r@{\hspace{2pt}}
		%
		@{\hspace{5pt}}r@{\hspace{5pt}}
		%
		@{\hspace{2pt}}r@{\hspace{2pt}}
	         @{\hspace{2pt}}r@{\hspace{2pt}}
		%
		@{\hspace{5pt}}r@{\hspace{5pt}}
		%
		@{\hspace{2pt}}r@{\hspace{2pt}}
		@{\hspace{2pt}}r@{\hspace{2pt}}
		%
		@{\hspace{5pt}}r@{\hspace{5pt}}
		%
		@{\hspace{2pt}}r@{\hspace{2pt}}
		@{\hspace{2pt}}r@{\hspace{2pt}}
		%
		@{\hspace{5pt}}r@{\hspace{5pt}}
		%
		@{\hspace{2pt}}r@{\hspace{2pt}}
		@{\hspace{2pt}}r@{\hspace{2pt}}
		%
		@{\hspace{5pt}}r@{\hspace{5pt}}
		%
		@{\hspace{2pt}}r@{\hspace{2pt}}
		%@{\hspace{2pt}}r@{\hspace{2pt}}
		%@{\hspace{2pt}}r@{\hspace{2pt}}
		}
		\toprule
		\multirow{2}{*}{type} & \multirow{2}{*}{method} & \multicolumn{2}{c}{Vina S$\downarrow$} & & \multicolumn{2}{c}{Vina M$\downarrow$} & & \multicolumn{2}{c}{Vina D$\downarrow$} & & \multicolumn{2}{c}{{HA\%$\uparrow$}}  & & \multicolumn{2}{c}{QED$\uparrow$} & & \multicolumn{2}{c}{SA$\uparrow$} & & \multicolumn{2}{c}{Div$\uparrow$} & %& \multirow{2}{*}{SR\%$\uparrow$} & 
		& \multirow{2}{*}{time$\downarrow$} \\
	    \cmidrule{3-4}\cmidrule{6-7} \cmidrule{9-10} \cmidrule{12-13} \cmidrule{15-16} \cmidrule{18-19} \cmidrule{21-22}
		& & Avg. & Med. &  & Avg. & Med. &  & Avg. & Med. & & Avg. & Med.  & & Avg. & Med.  & & Avg. & Med.  & & Avg. & Med.  & & \\ %& & \\
		%\multirow{2}{*}{method} & \multirow{2}{*}{\#c\%} &  \multirow{2}{*}{\#u\%} &  \multirow{2}{*}{QED} & \multicolumn{3}{c}{$\nmax=50$} & & \multicolumn{2}{c}{$\nmax=1$}\\
		%\cmidrule(r){5-7} \cmidrule(r){8-10} 
		%& & & & \avgshapesim(std) & \avggraphsim(std  &  \diversity(std  & & \avgshapesim(std) & \avggraphsim(std \\
		\midrule
		- & Reference                          & -6.00 & -6.10 & &  -6.37 & -6.15 & &  -7.16 & -7.02 & & - & - & & 0.50 & 0.47 & &  0.74 & 0.75 & & - & - & %& 23.1 & 
		& - \\
		\midrule
		\multirow{4}{*}{PM} 
		& \AR & -5.55 & -5.43 & &  -6.00 & -5.71 & &  -6.56 & -6.45 & &  37.69 & 31.00 & &  0.51 & 0.50 & &  0.64 & 0.63 & & - & - & %& 7.0 & 
		& 7,789 \\
		& \pockettwomol   & -4.92 & -4.52 & &  -6.14 & -5.61 & &  -6.88 & -6.59 & &  48.00 & 51.00 & &  0.58 & 0.58 & &  \textbf{0.76} & \textbf{0.77} & &  0.69 & 0.71 &  %& 24.9 & 
		& 2,544 \\
		& \targetdiff     &-5.22 & -6.09 & &  -6.45 & -6.67 & &  -7.63 & -7.76 & &  57.57 & 58.27 & &  0.49 & 0.49 & &  0.59 & 0.58 & &  0.72 & 0.71 & % & 10.4 & 
		& 1,252 \\
		%& \decompdiffbeta                    & 63.03 & %-4.72 & -4.86 & & \textbf{-6.84} & \textbf{-6.91} & & \textbf{-8.85} & \textbf{-8.90} & &  \textbf{72.16} & \textbf{72.16} & &  0.36 & 0.36 & &  0.55 & 0.55 & & 0.59 & 0.59 & & 14.9 \\ 
		%-4.76 & -6.18 & &  \textbf{-6.86} & \textbf{-7.52} & &  \textbf{-8.85} & \textbf{-8.96} & &  \textbf{72.7} & \textbf{89.8} & &  0.36 & 0.34 & &  0.55 & 0.57 & & 0.59 & 0.59 & & 15.4 \\
		& \decompdiffref  & -4.96 & -5.11 & &  -5.83 & -5.84 & &  -6.81 & -6.96 & &  47.76 & 48.66 & &  0.52 & 0.52 & &  0.67 & 0.66 & &  0.72 & 0.72 &  %& 15.2 & 
		& 1,859 \\
		\midrule
%<<<<<<< HEAD
%		\method                           & 17.96 & 12.56 & & -1.73 & -3.93 & & -6.85 & -7.04 & & 42.4\% & 40.4\% & & \textbf{0.66} & \textbf{0.68} & & 0.68 & 0.68 & & - & - & & 16.8\% \\
%		\methodwithsguide          & - & - & & - & - & & - & - & & - & - & & - & - & & - & - & & - & - & & - \\
%		\methodwithpguide          & -5.36 & -5.48 & & -6.52 & -6.17 & & -7.61 & -7.64 & & 58.8\% & 57.6\% & & 0.64 & 0.66 & & 0.62 & 0.63 & & - & - & & 13.7\% \\
%		\methodwithsandpguide   & -5.66 & -5.61 & & -6.61 & -6.21 & & -7.58 & -7.59 & & 57.6\% & 58.4\% & & 0.63 & 0.65 & & 0.61 & 0.62 & & 0.67 & 0.67 & & 12.2\% \\
%=======
		%\multirow{2}{*}{PU} 
		%& \method                           %& 98.31 
		%& 17.96 & 12.56 & & -1.73 & -3.93 & & -6.85 & -7.04 & & 42.4 & 40.4 & & \textbf{0.66} & \textbf{0.68} & & 0.68 & 0.68 & & 0.72 & 0.74 & & 16.8 \\
		%& \methodwithsguide          %& 98.18 
		%& 1.13 & -0.18 & & -4.63 & -4.72 & & -6.92 & -7.19 & & 46.2 & 44.0 & & \textbf{0.66} & 0.67 & & 0.67 & 0.67 & & 0.71 & 0.73 & & 16.7 \\
		%\midrule
		\multirow{2}{*}{PC}
		& \methodwithpguide       & \underline{-6.28} & \underline{-6.29} & &  \underline{-7.06} & \underline{-6.95} & & \textbf{-7.86} & \textbf{-8.07} & & \underline{78.75} & \textbf{94.00} & & \textbf{0.76} & \textbf{0.78} & &  \underline{0.72} & \underline{0.72} & & 0.63 & 0.66 & %& 28.0 & 
		& 462 \\
		& \methodwithsandpguide   & \textbf{-6.53} & \textbf{-6.55} & &  \textbf{-7.19} & \textbf{-7.15} & & \underline{-7.84} & \textbf{-8.07} & &  \textbf{79.92} & \underline{93.00} & & \underline{0.75} & \underline{0.78} & &  0.70 & 0.71 & & 0.64 & 0.66 & %& 26.7 & 
		& 561 \\
%>>>>>>> a73749118ddcc260459f56890a7fef6265351e43
		\bottomrule
	\end{tabular}%
	\begin{tablenotes}[normal,flushleft]
		\begin{footnotesize}
	\item 
\!\!Columns represent: \ziqi{``Vina S'': the binding affinities between the initially generated poses of molecules and the protein pockets; 
		``Vina M'': the binding affinities between the poses after local structure minimization and the protein pockets;
		``Vina D'': the binding affinities between the poses determined by AutoDock Vina~\cite{Eberhardt2021} and the protein targets;
		``QED'': the drug-likeness score;
		``SA'': the synthesizability score;
		``Div'': the diversity among generated molecules;
		``time'': the time cost to generate molecules.}
		
		\par
		\par
		\end{footnotesize}
	\end{tablenotes}
	\end{scriptsize}
\end{threeparttable}
  \vspace{-10pt}    
\end{table*}


==> tables/overall_results_new.tex <==
\begin{table*}
	\centering
		\caption{{Overall Comparison on Shape-Conditioned Molecule Generation}}
	\label{tbl:overall}
	\begin{small}
\begin{threeparttable}
	\begin{tabular}{
		@{\hspace{0pt}}l@{\hspace{2pt}}
		%
		@{\hspace{3pt}}r@{\hspace{3pt}}
		@{\hspace{3pt}}r@{\hspace{3pt}}
		@{\hspace{3pt}}r@{\hspace{3pt}}
		%
		%
		@{\hspace{3pt}}r@{\hspace{3pt}}
		%
		@{\hspace{3pt}}r@{\hspace{3pt}}
		%
		@{\hspace{0pt}}c@{\hspace{0pt}}
		%
	    	@{\hspace{3pt}}c@{\hspace{3pt}}
		%
		@{\hspace{3pt}}c@{\hspace{3pt}}
		%
		@{\hspace{3pt}}c@{\hspace{3pt}}
		%
		}
		\toprule
		method & \#v\% & \#s\% & \#u\%  & \avgshapesim(std) & \avggraphsim(std) & & \maxshapesim(std) & \maxgraphsim(std) &  \diversity(std) \\
		%\multirow{2}{*}{method} & \multirow{2}{*}{\#c\%} &  \multirow{2}{*}{\#u\%} &  \multirow{2}{*}{QED} & \multicolumn{3}{c}{$\nmax=50$} & & \multicolumn{2}{c}{$\nmax=1$}\\
		%\cmidrule(r){5-7} \cmidrule(r){8-10} 
		%& & & & \avgshapesim(std) & \avggraphsim(std  &  \diversity(std  & & \avgshapesim(std) & \avggraphsim(std \\
		\midrule
		\dataset                              & 100.0  & 100.0 & 100.0  & 0.729 (0.039) & \textbf{0.226} (0.038) & & 0.807 (0.042) & 0.241 (0.087) & \textbf{0.759} (0.015)\\
		\squid ($\lambda$=0.3)      & 100.0  & 100.0 &   94.2  & 0.740 (0.083) & 0.349 (0.088) & & \textbf{0.909} (0.070) & 0.549 (0.243) & 0.677 (0.065) \\
		\squid ($\lambda$=1.0)      & 100.0  & 100.0 &   95.0  & 0.699 (0.069) & 0.235 (0.045) & & 0.851 (0.061) & 0.271 (0.096) & 0.744 (0.046) \\
		\method                              & 100.0 & 99.3 & 100.0 & 0.771 (0.039) & 0.229 (0.043) & & 0.862 (0.036) & \textbf{0.237} (0.066) & 0.750 (0.041) \\
		\methodwithsguide               & 99.9 & 99.2 & 100.0 & \textbf{0.824} (0.029) & 0.230 (0.045) & & 0.903 (0.027) & 0.244 (0.076) & 0.750 (0.046) \\
		%\midrule
		%\method (+bt)            & 100.0 & 98.0 & 100.0 & 0.742 & 0.772 (0.040) & 0.211 (0.033) & & 0.862 (0.036) & 0.211 (0.033) & 0.743 (0.043) \\
		%\methodwithguide (+bt)    & 99.8 & 98.0 & 100.0 & 0.736 & 0.814 (0.031) & 0.193 (0.042) & & 0.895 (0.029) & 0.193 (0.042) & 0.745 (0.045) \\
		%
		\bottomrule
	\end{tabular}%
	\begin{tablenotes}[normal,flushleft]
		\begin{footnotesize}
	\item 
\!\!Columns represent: \ziqi{``\#v\%'': the percentage of valid molecules; ``\#s\%'': the percentage of valid and connected molecules;}%``\#c\%": the percentage of connected molecules; 
``\#u\%'': the percentage of unique molecules;
``\qed'': the average drug-likeness of generated molecules;
``\avgshapesim/\avggraphsim'': the average of shape or graph similarities between the condition molecules and generated molecules; ``std": the standard deviation;
``\maxshapesim'': the maximum of shape similarities between the condition molecules and generated molecules;
``\maxgraphsim'': the graph similarities between the condition molecules and the molecules with the maximum shape similarities;
``\diversity'': the diversity among the generated molecules. \par
		\par
		\end{footnotesize}
	\end{tablenotes}
\end{threeparttable}
\end{small}
  \vspace{-10pt}    
\end{table*}


==> tables/overall_results_new2.tex <==
\begin{table*}[h]
	\centering
		\caption{Similarity Comparison on Shape-based Molecule Generation}
	\label{tbl:overall}
	\begin{small}
\begin{threeparttable}
	\begin{tabular}{
		@{\hspace{0pt}}l@{\hspace{5pt}}
		%
		@{\hspace{3pt}}l@{\hspace{3pt}}
		%
		@{\hspace{3pt}}r@{\hspace{8pt}}
		@{\hspace{3pt}}c@{\hspace{3pt}}
		%
		@{\hspace{3pt}}c@{\hspace{3pt}}
		@{\hspace{3pt}}c@{\hspace{3pt}}
		%
	    	@{\hspace{0pt}}c@{\hspace{0pt}}
		%
		@{\hspace{3pt}}c@{\hspace{3pt}}
		@{\hspace{3pt}}c@{\hspace{3pt}}
		%
		@{\hspace{3pt}}r@{\hspace{3pt}}
		}
		\toprule
		$\delta_g$  & method          & \#d\%$\uparrow$ & $\diversity_d$$\uparrow$(std) & \avgshapesim$\uparrow$(std) & \avggraphsim$\downarrow$(std) & & \maxshapesim$\uparrow$(std) & \maxgraphsim$\downarrow$(std)       & \#n\%$\uparrow$  \\ 
		\midrule
		%\multirow{5}{0.079\linewidth}%{\hspace{0pt}0.1} & \dataset   & 0.0             & 0.628(0.139)          & 0.567(0.068)          & 0.078(0.010)          &  & 0.588(0.086)          & 0.081(0.013)          & 4.7              \\
		%&  \squid($\lambda$=0.3) & 0.0             & 0.320(0.000)          & 0.420(0.163)          & \textbf{0.056}(0.032) &  & 0.461(0.170)          & \textbf{0.065}(0.033) & 1.4              \\
		%& \squid($\lambda$=1.0) & 0.0             & 0.414(0.177)          & 0.483(0.184)          & \underline{0.064}(0.030)  &  & 0.531(0.182)          & \underline{0.073}(0.029)  & 2.4              \\
		%& \method               & \underline{1.6}     & \textbf{0.857}(0.034) & \underline{0.773}(0.045)  & 0.086(0.011)          &  & \underline{0.791}(0.053)  & 0.087(0.012)          & \underline{5.1}      \\
		%& \methodwithsguide      & \textbf{3.7}    & \underline{0.833}(0.062)  & \textbf{0.812}(0.037) & 0.088(0.009)          &  & \textbf{0.835}(0.047) & 0.089(0.010)          & \textbf{6.2}     \\ 
		%\cmidrule{2-10}
		%& improv\% & - & 36.5$^*$ & 43.2$^*$ & -53.6$^*$ &  & 42.0$^*$ & -33.8$^*$ & 31.9$^*$  \\
		%\midrule
		\multirow{6}{0.059\linewidth}{\hspace{0pt}1.0} 
		& \dataset & 12.3 & 0.734(0.068) & 0.750(0.037) & \textbf{0.226}(0.038) & & 0.819(0.039) & \underline{0.242}(0.085) & \textbf{100.0} \\
		%& \dataset & 12.3            & 0.734(0.068)          & 0.768(0.037)          & \textbf{0.228}(0.042) &  & 0.819(0.039)          & \underline{0.242}(0.085)  & \textbf{100.0}   \\
			& \squid($\lambda$=0.3) & 31.3            & 0.617(0.095)          & 0.740(0.076)          & 0.349(0.088)          &  & \textbf{0.909}(0.065) & 0.547(0.245)          & \textbf{100.0}   \\
			& \squid($\lambda$=1.0) & 14.7            & 0.720(0.062)          & 0.699(0.064)          & 0.235(0.045)          &  & 0.851(0.057)          & 0.271(0.097)          & \textbf{100.0}   \\
			& \method               & \underline{32.4}    & \textbf{0.751}(0.048) & \underline{0.771}(0.039)  & \underline{0.229}(0.043)  &  & 0.862(0.036)          & \textbf{0.237}(0.066) & \underline{99.3}     \\
			& \methodwithsguide                & \textbf{71.0}   & \underline{0.748}(0.046)  & \textbf{0.824}(0.029) & 0.230(0.045)          &  & \underline{0.903}(0.027)  & 0.244(0.076)          & 99.2             \\
		\cmidrule{2-10}
		& improv\% &  126.8$^*$ & 2.3$^*$ & 9.9$^*$ & -1.3$^*$ &  & -0.7$^*$ & -2.1 & -0.7$^*$  \\
		\midrule
		\multirow{6}{0.059\linewidth}{\hspace{0pt}0.7} 
		& \dataset & 12.3 & 0.734(0.068) & 0.750(0.037) & \textbf{0.226}(0.038) & & 0.819(0.039) & \underline{0.240}(0.081) & \textbf{100.0} \\
		%& \dataset & 12.3            & 0.736(0.076)          & 0.768(0.037)          & \textbf{0.228}(0.042) &  & 0.819(0.039)          & \underline{0.242}(0.085)  & \textbf{100.0}   \\
			& \squid($\lambda$=0.3) & 27.5            & 0.633(0.085)          & 0.735(0.074)          & 0.328(0.070)          &  & \underline{0.900}(0.062)  & 0.435(0.143)          & 95.4             \\
			& \squid($\lambda$=1.0) & 14.6            & 0.720(0.061)          & 0.699(0.064)          & 0.234(0.045)          &  & 0.851(0.057)          & 0.268(0.090)          & \underline{99.9}     \\
			& \method               & \underline{32.4}    & \textbf{0.751}(0.048) & \underline{0.771}(0.039)  & \underline{0.229}(0.043)  &  & 0.862(0.036)          & \textbf{0.237}(0.066) & 99.3             \\
			& \methodwithsguide     & \textbf{71.0}   & \underline{0.748}(0.046)  & \textbf{0.824}(0.029) & 0.230(0.045)          &  & \textbf{0.903}(0.027) & 0.244(0.074)          & 99.2             \\ 
		\cmidrule{2-10}
		& improv\% &  158.2$^*$ & 2.3$^*$ & 9.9$^*$ & -1.3$^*$ &  & 0.3 & 1.3 & -0.7$^*$  \\
		\midrule
		\multirow{6}{0.059\linewidth}{\hspace{0pt}0.5} & \dataset & 12.2            & 0.734(0.068)          & 0.750(0.037)          & \textbf{0.225}(0.037) &  & 0.819(0.039)          & \textbf{0.236}(0.070)          & \textbf{100.0}   \\
			& \squid($\lambda$=0.3) & 21.8            & 0.649(0.080)          & 0.728(0.072)          & 0.301(0.054)          &  & \underline{0.888}(0.061)  & 0.355(0.088)          & 85.9             \\
			& \squid($\lambda$=1.0) & 14.4            & 0.721(0.061)          & 0.699(0.063)          & 0.233(0.043)          &  & 0.850(0.057)          & 0.263(0.080)          & \underline{99.5}     \\
			& \method               & \underline{32.3}    & \textbf{0.751}(0.048) & \underline{0.771}(0.039)  & \underline{0.229}(0.043)  &  & 0.862(0.036)          & \textbf{0.236}(0.065) & 99.2             \\
			& \methodwithsguide     & \textbf{70.9}   & \underline{0.748}(0.046)  & \textbf{0.824}(0.029) & \underline{0.229}(0.044)  &  & \textbf{0.903}(0.027) & \underline{0.242}(0.069)  & 99.0             \\ 
		\cmidrule{2-10}
		& improv\% & 225.2$^*$ & 2.3$^*$ & 9.9$^*$ & -1.8$^*$ &  & 1.7$^*$ & 0.0 & -0.8$^*$  \\
		\midrule
		\multirow{6}{0.059\linewidth}{\hspace{0pt}0.3} & \dataset                & 10.6            & 0.736(0.076)          & 0.745(0.037)          & \textbf{0.211}(0.026) &  & 0.815(0.039)          & \textbf{0.215}(0.047)          & \textbf{100.0}   \\
			& \squid($\lambda$=0.3) & 8.3             & 0.669(0.114)          & 0.709(0.076)          & 0.237(0.033)          &  & 0.841(0.070)          & 0.253(0.038)          & 45.5             \\
		    & \squid($\lambda$=1.0) & 11.2            & 0.728(0.068)          & 0.695(0.064)          & \underline{0.216}(0.034)  &  & 0.841(0.056)          & 0.231(0.047)          & 84.3             \\
			& \method               & \underline{28.4}    & \textbf{0.762}(0.040) & \underline{0.770}(0.039)  & 0.217(0.031)          &  & \underline{0.858}(0.038)  & \underline{0.220}(0.046) & \underline{87.1}     \\
			& \methodwithsguide     & \textbf{61.4}   & \underline{0.760}(0.036)  & \textbf{0.823}(0.029) & 0.217(0.032)          &  & \textbf{0.900}(0.028) & 0.223(0.048)  & 86.0             \\ 
		\cmidrule{2-10}
		& improv\% &  448.2$^*$ & 3.5$^*$ & 10.5$^*$ & -2.8$^*$ &  & 7.0$^*$ & -2.3$^*$ & -12.9$^*$  \\
		\bottomrule
	\end{tabular}%
	\begin{tablenotes}[normal,flushleft]
		\begin{footnotesize}
	\item 
\!\!Columns represent: \ziqi{``$\delta_g$'': the graph similarity constraint; 
``\#d\%'': the percentage of molecules that satisfy the graph similarity constraint and are with high \shapesim ($\shapesim>=0.8$);
``\diversity'': the diversity among the generated molecules;
``\avgshapesim/\avggraphsim'': the average of shape or graph similarities between the condition molecules and generated molecules with $\graphsim<=\delta_g$;
``\maxshapesim'': the maximum of shape similarities between the condition molecules and generated molecules with $\graphsim<=\delta_g$;
``\maxgraphsim'': the graph similarities between the condition molecules and the molecules with the maximum shape similarities and $\graphsim<=\delta_g$;
``\#n\%'': the percentage of molecules that satisfy the graph similarity constraint ($\graphsim<=\delta_g$).
%
``$\uparrow$'' represents higher values are better, and ``$\downarrow$'' represents lower values are better.
%
 Best values are in \textbf{bold}, and second-best values are \underline{underlined}. 
} 
\par
		\par
		\end{footnotesize}
	\end{tablenotes}
\end{threeparttable}
\end{small}
  \vspace{-10pt}    
\end{table*}

==> tables/overall_results_quality.tex <==
\begin{table*}
	\centering
		\caption{\ziqi{Comparison on Molecule Quality with Shape-Conditioned Molecule Generation Methods with Pocket Unknown}}
	\label{tbl:overall}
	\begin{small}
\begin{threeparttable}
	\begin{tabular}{
		@{\hspace{0pt}}l@{\hspace{14pt}}
		@{\hspace{0pt}}l@{\hspace{2pt}}
		%
		@{\hspace{0pt}}c@{\hspace{2pt}}
		%
		@{\hspace{3pt}}c@{\hspace{3pt}}
		@{\hspace{3pt}}c@{\hspace{3pt}}
		@{\hspace{3pt}}c@{\hspace{3pt}}
		@{\hspace{3pt}}c@{\hspace{3pt}}
		%
		%
		}
		\toprule
		group & metric & & \squid ($\lambda$=1.0) & \squid ($\lambda$=0.3) & \methodwithsguide &  \method  \\
		%\multirow{2}{*}{method} & \multirow{2}{*}{\#c\%} &  \multirow{2}{*}{\#u\%} &  \multirow{2}{*}{QED} & \multicolumn{3}{c}{$\nmax=50$} & & \multicolumn{2}{c}{$\nmax=1$}\\
		%\cmidrule(r){5-7} \cmidrule(r){8-10} 
		%& & & & \avgshapesim(std) & \avggraphsim(std  &  \diversity(std  & & \avgshapesim(std) & \avggraphsim(std \\
		\midrule
		\multirow{2}{*}{stability} & atom stability ($\uparrow$) & & 0.992 & 0.992 & 0.988 & \textbf{0.993} \\
		& molecule stability ($\uparrow$) & & \textbf{0.921} & \textbf{0.921} & 0.828 & 0.885\\
		\midrule
		\multirow{3}{*}{Drug-likeness} & QED ($\uparrow$)                   & &  \textbf{0.766}   &   0.760       &       0.751     &  0.755       \\
		& SA ($\uparrow$)                      & &  \textbf{0.813}   &  \textbf{0.813}       &       0.692     &  0.699       \\
		& Lipinski ($\uparrow$)               & & \textbf{4.980} & 4.979 & 4.975 & 4.967      \\
		\midrule
		\multirow{4}{*}{3D structures} & RMSD($\downarrow$)                 & & 0.908 &   0.896           &  \textbf{0.878}         &   0.894       \\
		& JS. bond lengths ($\downarrow$) &  &  0.462 & 0.449 & \textbf{0.431} & 0.437    \\
		& JS. bond angles ($\downarrow$) &  &  0.296 & 0.277 & 0.196 & \textbf{0.183}  \\
		& JS. dihedral angles ($\downarrow$) &  & 0.209 & 0.199 & 0.170 & \textbf{0.168}   \\
		\midrule
		\multirow{5}{*}{Bonds} & JS. \#bonds per atoms ($\downarrow$) &  &  0.322 & 0.280 & 0.181 & \textbf{0.178}   \\
		& JS. basic bond types ($\downarrow$) &  & 0.083 & \textbf{0.069} & 0.191 & 0.183  \\
		& JS. freq. bond types ($\downarrow$) &  & 0.130 & \textbf{0.123} & 0.254 & 0.245  \\
		& JS. freq. bond pairs ($\downarrow$) &    & 0.089 & \textbf{0.085} & 0.221 & 0.209 \\
		& JS. freq. bond triplets ($\downarrow$) &  & 0.114 & \textbf{0.097} & 0.223 & 0.211 \\
		\midrule
		\multirow{3}{*}{Rings} & JS. \#rings ($\downarrow$) &  & 0.319 & 0.271 & 0.051 & \textbf{0.039}  \\
		& JS. \#n-sized rings ($\downarrow$) &   & 0.090 & \textbf{0.070} & 0.113 & 0.104  \\
		& \#Intersecting rings ($\uparrow$) &  & 5 & \textbf{6} & 5 & 4 \\
		%\method (+bt)            & 100.0 & 98.0 & 100.0 & 0.742 & 0.772 (0.040) & 0.211 (0.033) & & 0.862 (0.036) & 0.211 (0.033) & 0.743 (0.043) \\
		%\methodwithguide (+bt)    & 99.8 & 98.0 & 100.0 & 0.736 & 0.814 (0.031) & 0.193 (0.042) & & 0.895 (0.029) & 0.193 (0.042) & 0.745 (0.045) \\
		%
		\bottomrule
	\end{tabular}%
	\begin{tablenotes}[normal,flushleft]
		\begin{footnotesize}
	\item 
\!\!Columns represent:  \todo{ziqi: the calculation of RMSD metric is a little bit time-consuming, as it requires the optimization of the force field. I will update the results later.}\par
		\par
		\end{footnotesize}
	\end{tablenotes}
\end{threeparttable}
\end{small}
  \vspace{-10pt}    
\end{table*}


==> tables/overall_results_quality0.1.tex <==
\begin{table*}
	\centering
		\caption{\ziqi{Comparison on Molecule Quality with Shape-Conditioned Molecule Generation Methods with Pocket Unknown ($\delta_g$=0.1)}}
	\label{tbl:overall_results_quality_01}
	\begin{small}
\begin{threeparttable}
	\begin{tabular}{
		@{\hspace{0pt}}l@{\hspace{14pt}}
		@{\hspace{0pt}}l@{\hspace{2pt}}
		%
		@{\hspace{4pt}}c@{\hspace{4pt}}
		%
		@{\hspace{3pt}}c@{\hspace{3pt}}
		@{\hspace{3pt}}c@{\hspace{3pt}}
		@{\hspace{3pt}}c@{\hspace{3pt}}
		@{\hspace{3pt}}c@{\hspace{3pt}}
		@{\hspace{3pt}}c@{\hspace{3pt}}
		%
		%
		}
		\toprule
		group & metric & & \dataset & \squid ($\lambda$=0.3) & \squid ($\lambda$=1.0)  &  \method & \methodwithsguide  \\
		%\multirow{2}{*}{method} & \multirow{2}{*}{\#c\%} &  \multirow{2}{*}{\#u\%} &  \multirow{2}{*}{QED} & \multicolumn{3}{c}{$\nmax=50$} & & \multicolumn{2}{c}{$\nmax=1$}\\
		%\cmidrule(r){5-7} \cmidrule(r){8-10} 
		%& & & & \avgshapesim(std) & \avggraphsim(std  &  \diversity(std  & & \avgshapesim(std) & \avggraphsim(std \\
		\midrule
		\multirow{2}{*}{stability}
		& atom stability ($\uparrow$) & & 0.993 & \textbf{1.000} & 0.998 & 0.997 & 0.993     \\
		& mol stability ($\uparrow$) & & 0.947 & \textbf{0.997} & 0.990 & 0.956 & 0.913     \\
		\midrule
		\multirow{3}{*}{Drug-likeness} 
		& QED ($\uparrow$) & & 0.751 & \textbf{0.788} & 0.769 & 0.754 & 0.743    \\
		& SA ($\uparrow$) & & 0.818 & \textbf{0.839} & 0.820 & 0.695 & 0.707    \\
		& Lipinski ($\uparrow$) & & \textbf{5.000} & 4.996 & 4.986 & 4.977 & 4.967    \\
		\midrule
		\multirow{4}{*}{3D structures} 
		& RMSD ($\downarrow$) & & \textbf{0.371} & 0.838 & 0.883 & 0.916 & 0.939    \\
		& JS. bond lengths ($\downarrow$) & & \textbf{0.383} & 0.457 & 0.477 & 0.436 & 0.428    \\
		& JS. bond angles ($\downarrow$) & & 0.240 & \textbf{0.085} & 0.089 & 0.209 & 0.221    \\
		& JS. dihedral angles ($\downarrow$) & & 0.277 & 0.199 & 0.209 & \textbf{0.168} & 0.170    \\
		\midrule
		\multirow{5}{*}{Bonds} 
		& JS. \#bonds per atoms ($\downarrow$) & & 0.482 & 0.309 & 0.343 & 0.272 & \textbf{0.186}    \\
		& JS. basic bond types ($\downarrow$) & & 0.081 & \textbf{0.041} & 0.081 & 0.177 & 0.183    \\
		& JS. freq. bond types ($\downarrow$) & & 0.257 & \textbf{0.123} & 0.130 & 0.245 & 0.254    \\
		& JS. freq. bond pairs ($\downarrow$) & & 0.240 & \textbf{0.085} & 0.089 & 0.209 & 0.221    \\
		& JS. freq. bond triplets ($\downarrow$) & & 0.235 & \textbf{0.097} & 0.114 & 0.211 & 0.223    \\
		\midrule
		\multirow{3}{*}{Rings} 
		& JS. \#rings ($\downarrow$) & & 0.457 & 0.292 & 0.347 & \textbf{0.081} & 0.096    \\
		& JS. \#n-sized rings ($\downarrow$) & & 0.129 & \textbf{0.088} & 0.093 & 0.095 & 0.100    \\
		& \#Intersecting rings ($\uparrow$) & & 5 & \textbf{6} & 5 & 4 & 5    \\
		%\method (+bt)            & 100.0 & 98.0 & 100.0 & 0.742 & 0.772 (0.040) & 0.211 (0.033) & & 0.862 (0.036) & 0.211 (0.033) & 0.743 (0.043) \\
		%\methodwithguide (+bt)    & 99.8 & 98.0 & 100.0 & 0.736 & 0.814 (0.031) & 0.193 (0.042) & & 0.895 (0.029) & 0.193 (0.042) & 0.745 (0.045) \\
		%
		\bottomrule
	\end{tabular}%
	\begin{tablenotes}[normal,flushleft]
		\begin{footnotesize}
	\item 
\!\!Columns represent:  \todo{ziqi: the calculation of RMSD metric is a little bit time-consuming, as it requires the optimization of the force field. I will update the results later.}\par
		\par
		\end{footnotesize}
	\end{tablenotes}
\end{threeparttable}
\end{small}
  \vspace{-10pt}    
\end{table*}


==> tables/overall_results_quality0.3.tex <==
\begin{table*}
	\centering
		\caption{\ziqi{Comparison on Molecule Quality with Shape-Conditioned Molecule Generation Methods with Pocket Unknown ($\delta_g$=0.3)}}
	\label{tbl:overall_results_quality_03}
	\begin{small}
\begin{threeparttable}
	\begin{tabular}{
		@{\hspace{0pt}}l@{\hspace{14pt}}
		@{\hspace{0pt}}l@{\hspace{2pt}}
		%
		@{\hspace{4pt}}c@{\hspace{4pt}}
		%
		%@{\hspace{3pt}}c@{\hspace{3pt}}
		@{\hspace{3pt}}c@{\hspace{3pt}}
		@{\hspace{3pt}}c@{\hspace{3pt}}
		@{\hspace{3pt}}c@{\hspace{3pt}}
		@{\hspace{3pt}}c@{\hspace{3pt}}
		%
		%
		}
		\toprule
		group & metric & 
        %& \dataset 
        & \squid ($\lambda$=0.3) & \squid ($\lambda$=1.0)  &  \method & \methodwithsguide  \\
		%\multirow{2}{*}{method} & \multirow{2}{*}{\#c\%} &  \multirow{2}{*}{\#u\%} &  \multirow{2}{*}{QED} & \multicolumn{3}{c}{$\nmax=50$} & & \multicolumn{2}{c}{$\nmax=1$}\\
		%\cmidrule(r){5-7} \cmidrule(r){8-10} 
		%& & & & \avgshapesim(std) & \avggraphsim(std  &  \diversity(std  & & \avgshapesim(std) & \avggraphsim(std \\
		\midrule
		\multirow{2}{*}{stability}
		& atom stability ($\uparrow$) & 
        %& 0.990 
        & \textbf{0.993} & \textbf{0.993} & \textbf{0.993} & 0.989     \\
		& molecule stability ($\uparrow$) & 
        %& 0.877 
        & \textbf{0.930} & \textbf{0.930} & 0.894 & 0.842     \\
		\midrule
		\multirow{3}{*}{Drug-likeness} 
		& QED ($\uparrow$) & 
        %& \textbf{0.807} 
        & \textbf{0.766} & 0.760 & 0.755 & 0.752    \\
		& SA ($\uparrow$) & 
        %& \textbf{0.875} 
        & \textbf{0.817} & 0.814 & 0.699 & 0.692    \\
		& Lipinski ($\uparrow$) & 
        %& \textbf{4.999} 
        & \textbf{4.980} & 4.979 & 4.967 & 4.975    \\
		\midrule
		\multirow{4}{*}{3D structures} 
		& RMSD ($\downarrow$) & 
        %& \textbf{0.421} 
        & 0.892 & 0.909 & 0.896 & \textbf{0.881}    \\
		& JS. bond lengths ($\downarrow$) & 
        %& \textbf{0.287} 
        & 0.457 & 0.477 & 0.436 & \textbf{0.428}    \\
		& JS. bond angles ($\downarrow$) & 
        %& \textbf{0.079} 
        & \textbf{0.085} & 0.089 & 0.209 & 0.221    \\
		& JS. dihedral angles ($\downarrow$) & 
        %& \textbf{0.154} 
        & 0.199 & 0.209 & \textbf{0.168} & 0.170    \\
		\midrule
		\multirow{5}{*}{Bonds} 
		& JS. \#bonds per atoms ($\downarrow$) & 
        %& 0.330 
        & 0.281 & 0.320 & \textbf{0.180} & 0.183    \\
		& JS. basic bond types ($\downarrow$) & 
        %& \textbf{0.055} 
        & \textbf{0.066} & 0.082 & 0.184 & 0.191    \\
		& JS. freq. bond types ($\downarrow$) & 
        %& \textbf{0.090} 
        & \textbf{0.123} & 0.130 & 0.245 & 0.254    \\
		& JS. freq. bond pairs ($\downarrow$) & 
        %& \textbf{0.079} 
        & \textbf{0.085} & 0.089 & 0.209 & 0.221    \\
		& JS. freq. bond triplets ($\downarrow$) & 
        %& \textbf{0.089} 
        & \textbf{0.097} & 0.114 & 0.211 & 0.223    \\
		\midrule
		\multirow{3}{*}{Rings} 
		& JS. \#rings ($\downarrow$) & 
        %& 0.160 
        & 0.271 & 0.317 & \textbf{0.039} & 0.050    \\
		& JS. \#n-sized rings ($\downarrow$) & 
        %& \textbf{0.058} 
        & \textbf{0.073} & 0.089 & 0.104 & 0.113    \\
		& \#Intersecting rings ($\uparrow$) & 
        %& \textbf{6} 
        & \textbf{6} & 5 & 4 & 5    \\
		%\method (+bt)            & 100.0 & 98.0 & 100.0 & 0.742 & 0.772 (0.040) & 0.211 (0.033) & & 0.862 (0.036) & 0.211 (0.033) & 0.743 (0.043) \\
		%\methodwithguide (+bt)    & 99.8 & 98.0 & 100.0 & 0.736 & 0.814 (0.031) & 0.193 (0.042) & & 0.895 (0.029) & 0.193 (0.042) & 0.745 (0.045) \\
		%
		\bottomrule
	\end{tabular}%
	\begin{tablenotes}[normal,flushleft]
		\begin{footnotesize}
	\item 
\!\!Columns represent:  \todo{ziqi: the calculation of RMSD metric is a little bit time-consuming, as it requires the optimization of the force field. I will update the results later.}\par
		\par
		\end{footnotesize}
	\end{tablenotes}
\end{threeparttable}
\end{small}
  \vspace{-10pt}    
\end{table*}


==> tables/overall_results_validity.tex <==
\begin{table*}
\centering
\caption{{Overall Comparison on Shape-Conditioned Molecule Generation}}
\label{tbl:overall_results_validity}
\begin{small}
	\begin{threeparttable}
		\begin{tabular}{
				@{\hspace{0pt}}l@{\hspace{2pt}}
				%
				@{\hspace{3pt}}r@{\hspace{3pt}}
				@{\hspace{3pt}}r@{\hspace{3pt}}
				%
			}
			\toprule
			method & \#v\% & \#s\%  \\
			%\multirow{2}{*}{method} & \multirow{2}{*}{\#c\%} &  \multirow{2}{*}{\#u\%} &  \multirow{2}{*}{QED} & \multicolumn{3}{c}{$\nmax=50$} & & \multicolumn{2}{c}{$\nmax=1$}\\
			%\cmidrule(r){5-7} \cmidrule(r){8-10} 
			%& & & & \avgshapesim(std) & \avggraphsim(std  &  \diversity(std  & & \avgshapesim(std) & \avggraphsim(std \\
			\midrule
			\dataset                    & \textbf{100.0}  & \textbf{100.0} \\
			\squid ($\lambda$=0.3)      & \textbf{100.0}  & \textbf{100.0}  \\
			\squid ($\lambda$=1.0)      & \textbf{100.0}  & \textbf{100.0} \\
			\method                     & \textbf{100.0} & 99.3 \\
			\methodwithsguide           & 99.9 & 99.2 \\
			%\midrule
			%\method (+bt)            & 100.0 & 98.0 & 100.0 & 0.742 & 0.772 (0.040) & 0.211 (0.033) & & 0.862 (0.036) & 0.211 (0.033) & 0.743 (0.043) \\
			%\methodwithguide (+bt)    & 99.8 & 98.0 & 100.0 & 0.736 & 0.814 (0.031) & 0.193 (0.042) & & 0.895 (0.029) & 0.193 (0.042) & 0.745 (0.045) \\
			%
			\bottomrule
		\end{tabular}%
		\begin{tablenotes}[normal,flushleft]
			\begin{footnotesize}
				\item 
				\!\!Columns represent: \ziqi{``\#v\%'': the percentage of valid molecules; ``\#s\%'': the percentage of valid and connected molecules;} \par
				\par
			\end{footnotesize}
		\end{tablenotes}
	\end{threeparttable}
\end{small}
\vspace{-10pt}    
\end{table*}

